Dynamic Fractional Resource Scheduling vs. Batch Scheduling

We propose a novel job scheduling approach for homogeneous cluster computing platforms. Its key feature is the use of virtual machine technology to share fractional node resources in a precise and controlled manner. Other VM-based scheduling approaches have focused primarily on technical issues or on extensions to existing batch scheduling systems, while we take a more aggressive approach and seek to find heuristics that maximize an objective metric correlated with job performance. We derive absolute performance bounds and develop algorithms for the online, non-clairvoyant version of our scheduling problem. We further evaluate these algorithms in simulation against both synthetic and real-world HPC workloads and compare our algorithms to standard batch scheduling approaches. We find that our approach improves over batch scheduling by orders of magnitude in terms of job stretch, while leading to comparable or better resource utilization. Our results demonstrate that virtualization technology coupled with lightweight online scheduling strategies can afford dramatic improvements in performance for executing HPC workloads.

==> tabledata/costs-lubscaled-128-sload-gte-7-0-delay.tex <==
\greedy\activeres/opt=avg&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)\\
\greedy\activeres/\periodic/opt=avg&0.31/(1.09)&0.22/(0.54)&14.69/(51.48)&43.88/(92.52)&1.44/(7.98)&3.60/(8.42)\\
\greedy\activeres/\periodic/opt=avg/mft=300&0.31/(1.09)&0.21/(0.52)&14.74/(51.48)&41.70/(92.16)&1.44/(7.83)&3.46/(8.43)\\
\greedy\activeres/\periodic/opt=avg/mft=600&0.31/(1.10)&0.20/(0.51)&14.69/(51.84)&40.94/(88.20)&1.43/(7.79)&3.40/(7.96)\\
\greedy\activeres/\periodic/opt=avg/mvt=300&0.30/(1.11)&0.20/(0.52)&14.60/(50.40)&40.80/(89.64)&1.43/(7.70)&3.39/(8.04)\\
\greedy\activeres/\periodic/opt=avg/mvt=600&0.30/(1.06)&0.19/(0.48)&14.49/(51.12)&39.31/(88.92)&1.42/(7.58)&3.28/(7.82)\\
\greedy\activeres/opt=min&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)&0.00/(0.00)\\
\greedy\activeres/\periodic/opt=min&0.33/(1.11)&0.22/(0.52)&15.97/(61.20)&46.06/(109.08)&1.57/(8.66)&3.78/(9.49)\\
\greedy\activeres/\periodic/opt=min/mft=300&0.33/(1.12)&0.21/(0.53)&16.00/(60.84)&43.88/(106.56)&1.58/(8.66)&3.64/(9.26)\\
\greedy\activeres/\periodic/opt=min/mft=600&0.33/(1.10)&0.20/(0.51)&15.96/(60.84)&42.99/(105.48)&1.57/(8.76)&3.58/(9.21)\\
\greedy\activeres/\periodic/opt=min/mvt=300&0.33/(1.10)&0.20/(0.51)&15.93/(61.92)&42.78/(102.60)&1.57/(8.64)&3.56/(9.05)\\
\greedy\activeres/\periodic/opt=min/mvt=600&0.33/(1.10)&0.19/(0.48)&15.80/(60.48)&41.27/(98.28)&1.56/(8.75)&3.45/(8.60)\\
\greedy/\periodic/opt=avg&0.31/(0.88)&0.17/(0.50)&19.18/(55.80)&30.94/(90.36)&2.04/(8.65)&2.63/(8.25)\\
\greedy/\periodic/opt=avg/mft=300&0.31/(0.90)&0.16/(0.48)&19.27/(54.00)&28.84/(91.08)&2.05/(8.52)&2.48/(8.06)\\
\greedy/\periodic/opt=avg/mft=600&0.31/(0.91)&0.15/(0.48)&19.29/(54.72)&27.83/(87.84)&2.05/(8.53)&2.40/(7.95)\\
\greedy/\periodic/opt=avg/mvt=300&0.31/(0.90)&0.15/(0.48)&19.36/(55.08)&27.92/(86.40)&2.06/(8.74)&2.40/(7.93)\\
\greedy/\periodic/opt=avg/mvt=600&0.31/(0.91)&0.14/(0.47)&19.37/(54.36)&26.59/(86.40)&2.06/(9.07)&2.30/(7.64)\\
\greedy/\periodic/opt=min&0.32/(0.92)&0.17/(0.50)&20.23/(58.32)&31.59/(91.80)&2.14/(8.75)&2.69/(8.49)\\
\greedy/\periodic/opt=min/mft=300&0.32/(0.93)&0.16/(0.50)&20.34/(57.96)&29.55/(91.44)&2.15/(8.97)&2.54/(8.44)\\
\greedy/\periodic/opt=min/mft=600&0.32/(0.94)&0.15/(0.50)&20.34/(58.68)&28.62/(90.72)&2.15/(8.83)&2.47/(8.37)\\
\greedy/\periodic/opt=min/mvt=300&0.32/(0.92)&0.15/(0.49)&20.35/(58.32)&28.75/(89.28)&2.16/(9.10)&2.48/(8.27)\\
\greedy/\periodic/opt=min/mvt=600&0.32/(0.93)&0.14/(0.47)&20.55/(57.60)&27.24/(86.76)&2.18/(8.70)&2.36/(8.06)\\
\greedyp\activeres/opt=avg&0.06/(0.15)&0.00/(0.00)&5.49/(19.44)&0.00/(0.00)&0.55/(1.99)&0.00/(0.00)\\
\greedyp\activeres/\periodic/opt=avg&0.39/(1.30)&0.21/(0.49)&23.28/(73.80)&43.55/(92.88)&2.16/(9.39)&3.57/(8.29)\\
\greedyp\activeres/\periodic/opt=avg/mft=300&0.39/(1.30)&0.20/(0.50)&23.41/(73.80)&40.96/(89.28)&2.18/(9.41)&3.39/(8.14)\\
\greedyp\activeres/\periodic/opt=avg/mft=600&0.39/(1.27)&0.20/(0.49)&23.32/(73.80)&40.23/(87.84)&2.17/(9.39)&3.34/(7.99)\\
\greedyp\activeres/\periodic/opt=avg/mvt=300&0.38/(1.24)&0.19/(0.49)&23.08/(71.64)&40.23/(88.20)&2.15/(9.52)&3.34/(8.11)\\
\greedyp\activeres/\periodic/opt=avg/mvt=600&0.38/(1.24)&0.18/(0.46)&22.83/(72.36)&38.59/(82.80)&2.13/(9.46)&3.22/(7.73)\\
\greedyp\activeres/opt=min&0.06/(0.18)&0.00/(0.00)&5.37/(20.16)&0.00/(0.00)&0.54/(2.02)&0.00/(0.00)\\
\greedyp\activeres/\periodic/opt=min&0.41/(1.30)&0.21/(0.51)&24.24/(79.56)&45.64/(106.20)&2.27/(10.43)&3.74/(9.46)\\
\greedyp\activeres/\periodic/opt=min/mft=300&0.41/(1.29)&0.20/(0.51)&24.28/(80.64)&43.18/(103.68)&2.28/(10.45)&3.58/(9.03)\\
\greedyp\activeres/\periodic/opt=min/mft=600&0.41/(1.28)&0.20/(0.48)&24.34/(81.72)&42.24/(105.12)&2.29/(10.58)&3.52/(9.14)\\
\greedyp\activeres/\periodic/opt=min/mvt=300&0.41/(1.26)&0.19/(0.48)&24.19/(81.00)&42.15/(103.32)&2.28/(10.43)&3.51/(9.02)\\
\greedyp\activeres/\periodic/opt=min/mvt=600&0.40/(1.24)&0.18/(0.49)&23.98/(81.36)&40.49/(95.04)&2.26/(10.41)&3.39/(8.45)\\
\greedyp/\periodic/opt=avg&0.33/(0.95)&0.16/(0.47)&20.08/(55.80)&30.02/(92.52)&2.13/(8.38)&2.56/(8.08)\\
\greedyp/\periodic/opt=avg/mft=300&0.33/(0.95)&0.15/(0.46)&20.07/(55.08)&27.73/(88.56)&2.13/(8.97)&2.39/(7.62)\\
\greedyp/\periodic/opt=avg/mft=600&0.33/(0.91)&0.14/(0.46)&20.05/(54.36)&26.97/(86.40)&2.13/(8.50)&2.33/(7.70)\\
\greedyp/\periodic/opt=avg/mvt=300&0.33/(0.92)&0.14/(0.45)&20.09/(56.16)&27.08/(84.24)&2.13/(8.40)&2.34/(7.65)\\
\greedyp/\periodic/opt=avg/mvt=600&0.33/(0.92)&0.13/(0.44)&20.09/(55.80)&25.80/(83.88)&2.14/(8.50)&2.24/(7.38)\\
\greedyp/\periodic/opt=min&0.34/(0.96)&0.16/(0.49)&21.05/(59.04)&30.74/(91.44)&2.22/(9.11)&2.63/(8.47)\\
\greedyp/\periodic/opt=min/mft=300&0.34/(0.97)&0.15/(0.49)&21.07/(59.40)&28.29/(88.20)&2.23/(8.66)&2.44/(8.20)\\
\greedyp/\periodic/opt=min/mft=600&0.34/(0.97)&0.14/(0.48)&21.06/(58.32)&27.58/(88.20)&2.23/(8.85)&2.39/(8.20)\\
\greedyp/\periodic/opt=min/mvt=300&0.34/(0.97)&0.14/(0.47)&21.16/(59.40)&27.81/(85.68)&2.24/(9.37)&2.41/(7.89)\\
\greedyp/\periodic/opt=min/mvt=600&0.35/(0.99)&0.13/(0.46)&21.23/(60.12)&26.33/(82.80)&2.26/(9.57)&2.29/(7.56)\\
\greedypm\activeres/opt=avg&0.03/(0.08)&0.02/(0.06)&2.18/(9.00)&3.60/(15.12)&0.22/(1.12)&0.34/(1.16)\\
\greedypm\activeres/\periodic/opt=avg&0.36/(1.25)&0.23/(0.53)&19.48/(61.92)&47.73/(100.08)&1.86/(9.01)&3.90/(8.89)\\
\greedypm\activeres/\periodic/opt=avg/mft=300&0.36/(1.22)&0.21/(0.52)&19.34/(62.28)&45.39/(95.76)&1.85/(8.90)&3.75/(8.63)\\
\greedypm\activeres/\periodic/opt=avg/mft=600&0.36/(1.23)&0.21/(0.50)&19.35/(62.28)&44.58/(96.84)&1.85/(8.97)&3.69/(8.49)\\
\greedypm\activeres/\periodic/opt=avg/mvt=300&0.35/(1.21)&0.21/(0.49)&19.07/(60.84)&44.65/(95.40)&1.83/(8.70)&3.70/(8.40)\\
\greedypm\activeres/\periodic/opt=avg/mvt=600&0.35/(1.18)&0.20/(0.49)&18.81/(59.76)&43.22/(88.92)&1.81/(8.83)&3.59/(8.00)\\
\greedypm\activeres/opt=min&0.03/(0.07)&0.01/(0.06)&2.10/(9.72)&3.55/(14.40)&0.21/(1.19)&0.34/(1.24)\\
\greedypm\activeres/\periodic/opt=min&0.39/(1.25)&0.23/(0.52)&20.49/(73.08)&49.87/(114.12)&1.97/(10.17)&4.08/(9.91)\\
\greedypm\activeres/\periodic/opt=min/mft=300&0.39/(1.24)&0.21/(0.52)&20.52/(74.52)&47.36/(115.20)&1.98/(9.80)&3.91/(10.04)\\
\greedypm\activeres/\periodic/opt=min/mft=600&0.38/(1.22)&0.21/(0.51)&20.42/(73.08)&46.51/(110.88)&1.97/(9.78)&3.86/(9.64)\\
\greedypm\activeres/\periodic/opt=min/mvt=300&0.38/(1.21)&0.21/(0.50)&20.19/(74.16)&46.39/(106.56)&1.95/(9.82)&3.85/(9.32)\\
\greedypm\activeres/\periodic/opt=min/mvt=600&0.38/(1.19)&0.20/(0.48)&19.99/(73.80)&44.99/(101.88)&1.94/(9.70)&3.74/(9.15)\\
\greedypm/\periodic/opt=avg&0.32/(0.92)&0.17/(0.51)&19.30/(55.44)&31.90/(96.12)&2.06/(8.72)&2.69/(8.49)\\
\greedypm/\periodic/opt=avg/mft=300&0.32/(0.92)&0.16/(0.47)&19.33/(55.80)&29.56/(93.24)&2.07/(8.54)&2.52/(7.76)\\
\greedypm/\periodic/opt=avg/mft=600&0.32/(0.93)&0.15/(0.48)&19.38/(55.08)&28.75/(93.24)&2.08/(9.03)&2.46/(8.12)\\
\greedypm/\periodic/opt=avg/mvt=300&0.32/(0.93)&0.15/(0.46)&19.38/(57.24)&28.85/(92.88)&2.08/(8.76)&2.46/(7.84)\\
\greedypm/\periodic/opt=avg/mvt=600&0.32/(0.92)&0.14/(0.44)&19.47/(56.16)&27.27/(87.12)&2.09/(8.65)&2.35/(7.35)\\
\greedypm/\periodic/opt=min&0.34/(0.97)&0.17/(0.51)&20.37/(58.32)&32.38/(93.96)&2.17/(8.59)&2.74/(8.58)\\
\greedypm/\periodic/opt=min/mft=300&0.34/(0.96)&0.15/(0.49)&20.38/(58.32)&30.03/(91.44)&2.18/(8.67)&2.57/(8.58)\\
\greedypm/\periodic/opt=min/mft=600&0.34/(0.98)&0.15/(0.50)&20.36/(59.76)&29.26/(91.80)&2.17/(8.74)&2.51/(8.34)\\
\greedypm/\periodic/opt=min/mvt=300&0.34/(0.97)&0.15/(0.48)&20.50/(57.96)&29.23/(91.08)&2.19/(9.16)&2.51/(8.26)\\
\greedypm/\periodic/opt=min/mvt=600&0.34/(0.95)&0.14/(0.47)&20.50/(58.32)&27.99/(90.00)&2.19/(8.66)&2.41/(8.06)\\
\mcb\activeres/opt=avg&0.31/(1.42)&0.79/(2.35)&18.34/(77.40)&264.70/(1,054.44)&1.71/(7.28)&18.66/(44.70)\\
\mcb\activeres/opt=avg/mft=300&0.30/(1.37)&0.69/(2.06)&18.09/(74.52)&225.85/(806.04)&1.68/(6.95)&16.29/(41.64)\\
\mcb\activeres/opt=avg/mft=600&0.30/(1.20)&0.64/(1.86)&18.22/(86.76)&211.11/(731.16)&1.69/(7.05)&15.43/(36.75)\\
\mcb\activeres/opt=avg/mvt=300&0.30/(1.30)&0.60/(1.94)&17.86/(79.20)&203.01/(704.16)&1.66/(7.23)&14.86/(39.03)\\
\mcb\activeres/opt=avg/mvt=600&0.29/(1.25)&0.55/(1.71)&17.85/(74.52)&185.83/(602.64)&1.67/(7.49)&13.80/(37.68)\\
\mcb\activeres/\periodic/opt=avg&0.65/(2.40)&0.87/(2.47)&38.94/(136.08)&273.09/(1,051.92)&3.92/(15.05)&19.45/(48.50)\\
\mcb\activeres/\periodic/opt=avg/mft=300&0.64/(2.36)&0.76/(2.33)&38.72/(133.20)&231.89/(813.96)&3.89/(15.38)&16.95/(46.24)\\
\mcb\activeres/\periodic/opt=avg/mft=600&0.63/(2.30)&0.71/(2.23)&38.27/(133.20)&217.19/(739.44)&3.87/(15.66)&16.01/(43.44)\\
\mcb\activeres/\periodic/opt=avg/mvt=300&0.63/(2.29)&0.68/(2.14)&38.13/(131.04)&211.66/(709.92)&3.86/(15.20)&15.69/(42.54)\\
\mcb\activeres/\periodic/opt=avg/mvt=600&0.62/(2.22)&0.62/(2.07)&37.88/(129.24)&191.42/(659.52)&3.86/(14.99)&14.34/(41.70)\\
\mcb\activeres/opt=min&0.33/(1.37)&0.81/(2.55)&18.98/(79.92)&272.55/(1,056.60)&1.77/(7.66)&19.31/(44.88)\\
\mcb\activeres/opt=min/mft=300&0.31/(1.44)&0.70/(2.19)&18.60/(74.16)&232.88/(821.52)&1.74/(8.18)&16.92/(41.55)\\
\mcb\activeres/opt=min/mft=600&0.31/(1.53)&0.66/(2.32)&18.60/(78.12)&217.22/(733.32)&1.73/(8.33)&15.92/(40.13)\\
\mcb\activeres/opt=min/mvt=300&0.31/(1.46)&0.63/(2.14)&18.84/(75.96)&210.39/(711.72)&1.75/(7.64)&15.49/(38.93)\\
\mcb\activeres/opt=min/mvt=600&0.30/(1.30)&0.56/(2.01)&18.23/(71.64)&188.87/(616.32)&1.71/(8.24)&14.01/(36.32)\\
\mcb\activeres/\periodic/opt=min&0.68/(2.68)&0.89/(2.86)&40.76/(149.76)&281.85/(1,056.60)&4.09/(16.37)&20.18/(48.75)\\
\mcb\activeres/\periodic/opt=min/mft=300&0.68/(2.59)&0.78/(2.66)&40.58/(142.92)&240.06/(823.68)&4.09/(16.51)&17.63/(45.63)\\
\mcb\activeres/\periodic/opt=min/mft=600&0.67/(2.61)&0.73/(2.49)&40.26/(143.64)&223.68/(733.68)&4.06/(16.05)&16.56/(43.76)\\
\mcb\activeres/\periodic/opt=min/mvt=300&0.67/(2.54)&0.70/(2.44)&40.51/(145.08)&217.58/(712.80)&4.08/(16.20)&16.16/(42.47)\\
\mcb\activeres/\periodic/opt=min/mvt=600&0.66/(2.45)&0.64/(2.29)&39.99/(139.68)&197.14/(675.72)&4.05/(16.27)&14.80/(40.81)\\
\mcb/\periodic/opt=avg&0.46/(1.57)&0.58/(1.61)&28.12/(88.20)&168.48/(639.36)&2.91/(10.78)&12.12/(28.55)\\
\mcb/\periodic/opt=avg/mft=300&0.46/(1.50)&0.51/(1.52)&28.06/(89.28)&141.46/(480.60)&2.91/(10.72)&10.47/(26.77)\\
\mcb/\periodic/opt=avg/mft=600&0.46/(1.50)&0.47/(1.44)&27.80/(86.76)&133.05/(438.84)&2.89/(10.47)&9.92/(25.78)\\
\mcb/\periodic/opt=avg/mvt=300&0.46/(1.45)&0.46/(1.45)&27.93/(85.32)&130.19/(430.20)&2.90/(10.60)&9.76/(25.30)\\
\mcb/\periodic/opt=avg/mvt=600&0.46/(1.46)&0.42/(1.42)&27.90/(84.24)&118.21/(407.16)&2.91/(10.82)&8.94/(24.22)\\
\mcb/\periodic/opt=min&0.48/(1.70)&0.59/(1.77)&29.27/(96.48)&173.79/(649.80)&3.03/(11.09)&12.55/(29.53)\\
\mcb/\periodic/opt=min/mft=300&0.48/(1.72)&0.51/(1.65)&29.26/(96.12)&145.58/(491.76)&3.03/(10.80)&10.83/(27.13)\\
\mcb/\periodic/opt=min/mft=600&0.48/(1.69)&0.49/(1.55)&29.20/(95.76)&137.30/(433.80)&3.03/(11.18)&10.30/(26.17)\\
\mcb/\periodic/opt=min/mvt=300&0.48/(1.63)&0.47/(1.50)&29.27/(93.60)&133.42/(417.24)&3.04/(11.29)&10.04/(25.24)\\
\mcb/\periodic/opt=min/mvt=600&0.48/(1.59)&0.43/(1.40)&29.19/(90.72)&121.07/(392.04)&3.04/(11.52)&9.21/(24.09)\\
/\periodic/opt=avg&0.31/(0.90)&0.17/(0.51)&20.10/(55.08)&31.06/(92.16)&2.15/(8.88)&2.71/(8.56)\\
/\periodic/opt=avg/mft=300&0.31/(0.89)&0.17/(0.50)&20.05/(54.36)&31.20/(91.44)&2.15/(8.73)&2.72/(8.51)\\
/\periodic/opt=avg/mft=600&0.31/(0.90)&0.17/(0.51)&20.09/(56.16)&31.10/(92.88)&2.15/(9.27)&2.71/(8.46)\\
/\periodic/opt=avg/mvt=300&0.31/(0.88)&0.16/(0.50)&20.11/(55.08)&30.30/(90.00)&2.16/(8.91)&2.65/(8.45)\\
/\periodic/opt=avg/mvt=600&0.31/(0.89)&0.16/(0.49)&20.22/(54.72)&29.19/(87.84)&2.18/(9.09)&2.57/(8.34)\\
/\periodic/opt=min&0.33/(0.92)&0.17/(0.53)&21.19/(57.60)&31.68/(95.40)&2.26/(8.94)&2.76/(8.90)\\
/\periodic/opt=min/mft=300&0.33/(0.92)&0.17/(0.53)&21.19/(57.60)&31.68/(95.40)&2.26/(8.94)&2.76/(8.90)\\
/\periodic/opt=min/mft=600&0.33/(0.92)&0.17/(0.53)&21.19/(57.60)&31.68/(95.40)&2.26/(8.94)&2.76/(8.90)\\
/\periodic/opt=min/mvt=300&0.33/(0.92)&0.16/(0.51)&21.19/(57.96)&30.99/(95.04)&2.26/(8.78)&2.72/(8.90)\\
/\periodic/opt=min/mvt=600&0.33/(0.92)&0.16/(0.51)&21.40/(58.32)&29.77/(93.24)&2.30/(9.11)&2.63/(8.76)\\
\mcbs/opt=avg&0.20/(0.59)&0.32/(0.69)&13.53/(32.76)&52.52/(126.00)&1.53/(6.36)&4.94/(11.92)\\
\mcbs/opt=avg/mft=300&0.20/(0.59)&0.32/(0.69)&13.51/(32.40)&52.53/(127.08)&1.53/(6.27)&4.94/(12.00)\\
\mcbs/opt=avg/mft=600&0.20/(0.60)&0.32/(0.69)&13.53/(32.76)&52.42/(126.72)&1.53/(6.17)&4.93/(11.98)\\
\mcbs/opt=avg/mvt=300&0.20/(0.58)&0.32/(0.69)&13.58/(33.48)&51.72/(126.72)&1.54/(6.35)&4.87/(12.08)\\
\mcbs/opt=avg/mvt=600&0.20/(0.58)&0.31/(0.68)&13.65/(32.40)&50.28/(125.28)&1.55/(6.04)&4.77/(11.94)\\
\mcbs/opt=max&0.20/(0.58)&0.33/(0.71)&13.25/(31.32)&56.16/(146.16)&1.50/(6.26)&5.32/(13.47)\\
\mcbs/opt=max/mft=300&0.20/(0.58)&0.33/(0.71)&13.25/(31.32)&56.16/(146.16)&1.50/(6.26)&5.32/(13.47)\\
\mcbs/opt=max/mft=600&0.20/(0.58)&0.33/(0.71)&13.25/(31.32)&56.16/(146.16)&1.50/(6.26)&5.32/(13.47)\\
\mcbs/opt=max/mvt=300&0.20/(0.58)&0.32/(0.70)&13.34/(32.04)&55.20/(145.80)&1.51/(6.32)&5.24/(13.42)\\
\mcbs/opt=max/mvt=600&0.20/(0.60)&0.31/(0.68)&13.42/(32.76)&53.64/(139.32)&1.52/(6.31)&5.12/(12.98)\\


==> tabledata/costs-lubscaled-128-sload-gte-7-300-delay.tex <==
\greedy\activeres/\optavg&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)\\
\greedy\activeres/\optmin&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)&0.00 (0.00)\\
\greedy/\periodic/\optavg&0.44 (1.02)&0.21 (0.63)&30.12 (75.96)&38.81 (124.56)&5.03 (21.58)&4.79 (18.26)\\
\greedy/\periodic/\optavg/\mft[300]&0.44 (1.04)&0.20 (0.62)&29.82 (75.24)&36.41 (110.88)&4.98 (21.52)&4.52 (15.80)\\
\greedy/\periodic/\optavg/\mft[600]&0.44 (1.03)&0.20 (0.62)&29.63 (75.96)&35.46 (112.32)&4.94 (20.66)&4.41 (16.26)\\
\greedy/\periodic/\optavg/\mvt[300]&0.44 (1.03)&0.20 (0.63)&29.69 (74.88)&35.46 (118.08)&4.95 (21.03)&4.40 (17.08)\\
\greedy/\periodic/\optavg/\mvt[600]&0.44 (1.04)&0.19 (0.60)&29.55 (74.52)&33.91 (107.64)&4.91 (21.01)&4.22 (15.65)\\
\greedy/\periodic/\optmin&0.48 (1.08)&0.21 (0.60)&32.58 (83.52)&38.79 (110.52)&5.41 (21.76)&4.81 (16.17)\\
\greedy/\periodic/\optmin/\mft[300]&0.47 (1.08)&0.20 (0.59)&32.28 (82.80)&36.23 (107.28)&5.36 (21.55)&4.52 (15.40)\\
\greedy/\periodic/\optmin/\mft[600]&0.47 (1.08)&0.19 (0.58)&32.18 (82.80)&35.15 (106.56)&5.33 (21.31)&4.39 (15.27)\\
\greedy/\periodic/\optmin/\mvt[300]&0.47 (1.06)&0.19 (0.57)&32.25 (82.80)&35.11 (103.68)&5.34 (21.83)&4.37 (15.21)\\
\greedy/\periodic/\optmin/\mvt[600]&0.47 (1.07)&0.18 (0.58)&32.04 (83.16)&33.60 (103.68)&5.29 (21.94)&4.20 (14.83)\\
\greedy\activeres/\periodic/\optavg&0.45 (1.28)&0.28 (0.69)&26.07 (73.08)&55.45 (126.00)&3.95 (20.26)&6.59 (17.29)\\
\greedy\activeres/\periodic/\optavg/\mft[300]&0.45 (1.27)&0.27 (0.66)&25.68 (71.64)&53.16 (119.16)&3.89 (19.76)&6.36 (16.62)\\
\greedy\activeres/\periodic/\optavg/\mft[600]&0.44 (1.26)&0.26 (0.67)&25.39 (71.28)&51.96 (117.36)&3.85 (19.57)&6.23 (16.52)\\
\greedy\activeres/\periodic/\optavg/\mvt[300]&0.44 (1.26)&0.26 (0.65)&25.23 (71.28)&51.74 (123.12)&3.81 (19.60)&6.18 (16.42)\\
\greedy\activeres/\periodic/\optavg/\mvt[600]&0.44 (1.26)&0.25 (0.65)&24.86 (70.56)&50.07 (120.24)&3.75 (19.24)&5.98 (16.01)\\
\greedy\activeres/\periodic/\optmin&0.50 (1.29)&0.27 (0.66)&29.27 (84.96)&58.06 (124.56)&4.49 (22.55)&6.94 (17.65)\\
\greedy\activeres/\periodic/\optmin/\mft[300]&0.50 (1.29)&0.26 (0.65)&28.74 (83.16)&55.46 (123.84)&4.41 (22.07)&6.66 (17.31)\\
\greedy\activeres/\periodic/\optmin/\mft[600]&0.50 (1.29)&0.26 (0.63)&28.58 (83.88)&54.32 (123.12)&4.38 (21.89)&6.55 (17.38)\\
\greedy\activeres/\periodic/\optmin/\mvt[300]&0.50 (1.27)&0.26 (0.63)&28.50 (83.52)&53.86 (120.96)&4.37 (21.71)&6.48 (17.26)\\
\greedy\activeres/\periodic/\optmin/\mvt[600]&0.49 (1.27)&0.24 (0.62)&28.08 (83.52)&51.97 (117.36)&4.29 (21.80)&6.25 (16.53)\\
\greedyp\activeres/\optavg&0.06 (0.17)&0.00 (0.00)&5.78 (20.52)&0.00 (0.00)&0.58 (2.09)&0.00 (0.00)\\
\greedyp\activeres/\optmin&0.06 (0.17)&0.00 (0.00)&5.67 (18.00)&0.00 (0.00)&0.57 (2.04)&0.00 (0.00)\\
\greedyp/\periodic/\optavg&0.46 (1.05)&0.20 (0.64)&30.86 (76.68)&37.70 (111.96)&5.16 (21.11)&4.67 (16.20)\\
\greedyp/\periodic/\optavg/\mft[300]&0.46 (1.07)&0.19 (0.61)&30.46 (74.88)&35.37 (108.72)&5.09 (21.05)&4.41 (15.45)\\
\greedyp/\periodic/\optavg/\mft[600]&0.46 (1.06)&0.19 (0.60)&30.31 (75.24)&34.51 (110.88)&5.05 (20.97)&4.32 (15.12)\\
\greedyp/\periodic/\optavg/\mvt[300]&0.46 (1.07)&0.19 (0.62)&30.39 (77.04)&34.63 (106.56)&5.06 (20.52)&4.33 (15.29)\\
\greedyp/\periodic/\optavg/\mvt[600]&0.46 (1.05)&0.18 (0.60)&30.17 (77.04)&33.08 (103.68)&5.02 (20.36)&4.14 (14.68)\\
\greedyp/\periodic/\optmin&0.50 (1.11)&0.20 (0.60)&33.34 (85.32)&37.52 (107.64)&5.54 (22.20)&4.67 (15.76)\\
\greedyp/\periodic/\optmin/\mft[300]&0.49 (1.11)&0.19 (0.58)&32.95 (83.88)&35.05 (104.40)&5.47 (21.45)&4.39 (15.09)\\
\greedyp/\periodic/\optmin/\mft[600]&0.49 (1.10)&0.18 (0.58)&32.79 (84.60)&34.07 (103.68)&5.45 (21.41)&4.28 (15.30)\\
\greedyp/\periodic/\optmin/\mvt[300]&0.49 (1.10)&0.18 (0.57)&32.88 (84.60)&34.17 (105.84)&5.46 (21.94)&4.29 (15.04)\\
\greedyp/\periodic/\optmin/\mvt[600]&0.49 (1.11)&0.18 (0.57)&32.70 (83.52)&32.74 (101.52)&5.41 (21.37)&4.11 (14.29)\\
\greedyp\activeres/\periodic/\optavg&0.53 (1.36)&0.28 (0.68)&37.08 (83.52)&56.42 (123.12)&5.37 (22.68)&6.78 (17.07)\\
\greedyp\activeres/\periodic/\optavg/\mft[300]&0.52 (1.35)&0.27 (0.69)&35.90 (84.96)&53.48 (123.12)&5.21 (22.27)&6.47 (17.30)\\
\greedyp\activeres/\periodic/\optavg/\mft[600]&0.52 (1.36)&0.26 (0.69)&35.58 (84.60)&52.38 (120.60)&5.17 (21.34)&6.35 (17.24)\\
\greedyp\activeres/\periodic/\optavg/\mvt[300]&0.52 (1.35)&0.26 (0.66)&35.33 (84.24)&52.26 (117.00)&5.12 (21.58)&6.32 (16.78)\\
\greedyp\activeres/\periodic/\optavg/\mvt[600]&0.51 (1.35)&0.25 (0.65)&34.70 (82.80)&50.41 (114.84)&5.03 (21.52)&6.09 (16.26)\\
\greedyp\activeres/\periodic/\optmin&0.58 (1.37)&0.28 (0.65)&39.67 (97.92)&58.56 (127.08)&5.87 (24.87)&7.09 (17.91)\\
\greedyp\activeres/\periodic/\optmin/\mft[300]&0.57 (1.38)&0.26 (0.65)&38.67 (98.28)&55.64 (124.20)&5.73 (23.92)&6.78 (17.45)\\
\greedyp\activeres/\periodic/\optmin/\mft[600]&0.57 (1.38)&0.26 (0.65)&38.39 (96.48)&54.46 (122.40)&5.69 (24.22)&6.65 (17.17)\\
\greedyp\activeres/\periodic/\optmin/\mvt[300]&0.57 (1.37)&0.25 (0.62)&38.27 (97.56)&53.82 (119.52)&5.66 (24.30)&6.54 (17.04)\\
\greedyp\activeres/\periodic/\optmin/\mvt[600]&0.56 (1.36)&0.24 (0.63)&37.70 (97.20)&52.14 (119.16)&5.56 (23.88)&6.34 (16.48)\\
\greedypm\activeres/\optavg&0.03 (0.08)&0.02 (0.05)&2.31 (9.72)&3.75 (14.04)&0.24 (1.11)&0.37 (1.18)\\
\greedypm\activeres/\optmin&0.03 (0.07)&0.02 (0.05)&2.25 (10.08)&3.69 (13.32)&0.23 (1.19)&0.36 (1.22)\\
\greedypm/\periodic/\optavg&0.46 (1.05)&0.21 (0.64)&30.36 (77.04)&39.63 (114.84)&5.11 (20.79)&4.88 (16.67)\\
\greedypm/\periodic/\optavg/\mft[300]&0.46 (1.05)&0.20 (0.64)&29.96 (75.24)&37.04 (114.12)&5.03 (20.61)&4.60 (15.78)\\
\greedypm/\periodic/\optavg/\mft[600]&0.45 (1.04)&0.20 (0.61)&29.79 (77.40)&36.13 (109.80)&5.01 (20.41)&4.50 (15.52)\\
\greedypm/\periodic/\optavg/\mvt[300]&0.45 (1.06)&0.20 (0.62)&29.90 (75.60)&36.03 (113.40)&5.02 (20.99)&4.48 (15.41)\\
\greedypm/\periodic/\optavg/\mvt[600]&0.45 (1.06)&0.19 (0.60)&29.70 (77.04)&34.83 (116.28)&4.98 (21.06)&4.33 (16.83)\\
\greedypm/\periodic/\optmin&0.49 (1.10)&0.21 (0.60)&32.93 (84.24)&39.21 (112.32)&5.52 (21.65)&4.85 (16.03)\\
\greedypm/\periodic/\optmin/\mft[300]&0.49 (1.10)&0.20 (0.61)&32.46 (84.60)&36.78 (108.36)&5.43 (21.97)&4.58 (15.71)\\
\greedypm/\periodic/\optmin/\mft[600]&0.49 (1.10)&0.19 (0.58)&32.34 (83.88)&35.87 (108.72)&5.41 (21.39)&4.49 (15.59)\\
\greedypm/\periodic/\optmin/\mvt[300]&0.49 (1.10)&0.19 (0.57)&32.44 (84.24)&35.78 (108.72)&5.42 (21.67)&4.45 (15.15)\\
\greedypm/\periodic/\optmin/\mvt[600]&0.49 (1.10)&0.18 (0.57)&32.24 (83.16)&34.31 (106.56)&5.37 (22.19)&4.28 (15.07)\\
\greedypm\activeres/\periodic/\optavg&0.51 (1.33)&0.29 (0.68)&32.78 (80.28)&60.90 (129.60)&4.88 (22.02)&7.30 (18.27)\\
\greedypm\activeres/\periodic/\optavg/\mft[300]&0.50 (1.33)&0.28 (0.69)&31.93 (81.00)&57.83 (123.48)&4.76 (21.49)&6.98 (17.71)\\
\greedypm\activeres/\periodic/\optavg/\mft[600]&0.50 (1.35)&0.27 (0.68)&31.57 (81.00)&56.72 (119.88)&4.70 (21.30)&6.85 (17.02)\\
\greedypm\activeres/\periodic/\optavg/\mvt[300]&0.49 (1.33)&0.27 (0.67)&31.19 (78.84)&56.59 (121.32)&4.65 (21.03)&6.81 (17.11)\\
\greedypm\activeres/\periodic/\optavg/\mvt[600]&0.49 (1.34)&0.26 (0.65)&30.60 (79.56)&54.88 (120.96)&4.55 (20.70)&6.61 (17.24)\\
\greedypm\activeres/\periodic/\optmin&0.56 (1.37)&0.29 (0.66)&35.78 (96.48)&62.95 (135.72)&5.42 (24.00)&7.59 (18.32)\\
\greedypm\activeres/\periodic/\optmin/\mft[300]&0.55 (1.36)&0.27 (0.66)&34.88 (95.04)&59.84 (132.48)&5.29 (23.42)&7.27 (18.23)\\
\greedypm\activeres/\periodic/\optmin/\mft[600]&0.55 (1.36)&0.27 (0.65)&34.45 (92.88)&58.68 (130.32)&5.23 (23.76)&7.14 (17.80)\\
\greedypm\activeres/\periodic/\optmin/\mvt[300]&0.55 (1.36)&0.27 (0.64)&34.25 (94.32)&58.31 (128.52)&5.19 (23.12)&7.07 (17.32)\\
\greedypm\activeres/\periodic/\optmin/\mvt[600]&0.54 (1.34)&0.26 (0.62)&33.80 (94.32)&56.45 (127.08)&5.11 (23.23)&6.84 (16.94)\\
\mcb\activeres/\optavg&0.38 (1.15)&1.16 (2.35)&56.54 (214.56)&470.14 (998.28)&6.10 (17.36)&55.01 (86.16)\\
\mcb\activeres/\optavg/\mft[300]&0.18 (0.99)&0.86 (2.98)&20.23 (162.72)&327.56 (1,313.64)&2.02 (14.26)&31.45 (80.96)\\
\mcb\activeres/\optavg/\mft[600]&0.14 (0.67)&0.73 (2.60)&12.86 (90.36)&279.56 (1,201.68)&1.31 (9.68)&25.24 (65.40)\\
\mcb\activeres/\optavg/\mvt[300]&0.13 (0.48)&0.61 (2.09)&10.04 (51.84)&238.86 (1,101.60)&1.03 (2.88)&20.89 (42.69)\\
\mcb\activeres/\optavg/\mvt[600]&0.12 (0.39)&0.53 (1.49)&9.27 (37.80)&206.62 (822.60)&0.97 (3.42)&18.17 (41.67)\\
\mcb\activeres/\optmin&0.42 (1.26)&1.17 (2.36)&61.66 (230.40)&490.48 (1,005.48)&6.67 (18.83)&57.46 (90.29)\\
\mcb\activeres/\optmin/\mft[300]&0.20 (0.98)&0.86 (2.89)&21.60 (174.96)&337.86 (1,343.16)&2.18 (15.58)&32.59 (89.17)\\
\mcb\activeres/\optmin/\mft[600]&0.15 (0.78)&0.75 (2.72)&13.24 (102.96)&291.29 (1,306.80)&1.37 (8.67)&26.28 (68.39)\\
\mcb\activeres/\optmin/\mvt[300]&0.13 (0.72)&0.63 (2.12)&10.25 (78.48)&247.80 (1,083.24)&1.06 (3.08)&21.73 (46.10)\\
\mcb\activeres/\optmin/\mvt[600]&0.13 (0.37)&0.53 (1.51)&9.51 (38.16)&212.16 (825.48)&1.00 (2.89)&18.68 (41.15)\\
\mcb/\periodic/\optavg&0.52 (1.07)&0.69 (2.92)&38.66 (83.52)&235.57 (1,181.88)&6.34 (25.03)&25.02 (41.57)\\
\mcb/\periodic/\optavg/\mft[300]&0.50 (1.05)&0.55 (2.14)&35.19 (80.28)&164.35 (798.48)&6.04 (24.52)&18.31 (36.68)\\
\mcb/\periodic/\optavg/\mft[600]&0.49 (1.04)&0.51 (1.66)&34.72 (79.56)&149.35 (709.92)&5.97 (24.57)&16.87 (35.67)\\
\mcb/\periodic/\optavg/\mvt[300]&0.49 (1.07)&0.47 (1.32)&34.57 (80.64)&139.75 (600.84)&5.94 (25.07)&15.76 (33.88)\\
\mcb/\periodic/\optavg/\mvt[600]&0.49 (1.06)&0.43 (1.18)&34.15 (78.48)&124.47 (480.24)&5.85 (24.90)&14.18 (33.19)\\
\mcb/\periodic/\optmin&0.56 (1.10)&0.69 (3.03)&41.59 (86.76)&243.13 (1,269.00)&6.83 (26.38)&25.74 (43.24)\\
\mcb/\periodic/\optmin/\mft[300]&0.54 (1.10)&0.55 (2.04)&38.09 (86.04)&167.67 (826.56)&6.51 (26.03)&18.75 (38.89)\\
\mcb/\periodic/\optmin/\mft[600]&0.53 (1.09)&0.51 (1.68)&37.47 (84.96)&151.97 (755.64)&6.42 (26.10)&17.23 (36.68)\\
\mcb/\periodic/\optmin/\mvt[300]&0.53 (1.11)&0.47 (1.40)&37.32 (86.40)&142.42 (619.92)&6.39 (26.37)&16.13 (36.79)\\
\mcb/\periodic/\optmin/\mvt[600]&0.53 (1.12)&0.43 (1.12)&36.93 (86.76)&126.13 (490.68)&6.30 (26.13)&14.45 (34.48)\\
\mcb\activeres/\periodic/\optavg&0.67 (1.08)&1.21 (2.54)&70.98 (163.44)&461.18 (1,045.44)&11.97 (26.78)&70.57 (106.14)\\
\mcb\activeres/\periodic/\optavg/\mft[300]&0.54 (1.05)&0.89 (3.12)&44.52 (128.52)&314.64 (1,351.80)&7.54 (26.28)&39.94 (105.55)\\
\mcb\activeres/\periodic/\optavg/\mft[600]&0.51 (1.03)&0.77 (2.69)&38.07 (83.52)&263.46 (1,245.60)&6.59 (24.99)&31.32 (78.30)\\
\mcb\activeres/\periodic/\optavg/\mvt[300]&0.50 (1.07)&0.65 (2.08)&35.99 (80.64)&222.61 (1,057.32)&6.24 (25.69)&25.53 (53.96)\\
\mcb\activeres/\periodic/\optavg/\mvt[600]&0.50 (1.09)&0.57 (1.53)&35.09 (77.04)&191.91 (795.24)&6.08 (25.58)&22.24 (50.41)\\
\mcb\activeres/\periodic/\optmin&0.72 (1.15)&1.21 (2.68)&77.04 (170.28)&479.31 (1,109.52)&13.01 (28.93)&73.61 (117.15)\\
\mcb\activeres/\periodic/\optmin/\mft[300]&0.58 (1.12)&0.89 (3.02)&47.63 (135.00)&325.09 (1,370.16)&8.11 (27.86)&41.44 (112.18)\\
\mcb\activeres/\periodic/\optmin/\mft[600]&0.55 (1.10)&0.77 (2.76)&41.08 (93.60)&271.59 (1,337.76)&7.13 (27.14)&32.52 (81.60)\\
\mcb\activeres/\periodic/\optmin/\mvt[300]&0.54 (1.11)&0.65 (2.16)&38.88 (86.40)&227.80 (1,129.32)&6.72 (27.27)&26.33 (54.97)\\
\mcb\activeres/\periodic/\optmin/\mvt[600]&0.54 (1.11)&0.56 (1.53)&37.94 (85.32)&194.57 (836.28)&6.57 (26.52)&22.55 (50.29)\\
/\periodic/\optavg&0.45 (1.02)&0.21 (0.64)&31.29 (76.32)&38.76 (113.76)&5.25 (22.34)&4.89 (16.87)\\
/\periodic/\optavg/\mft[300]&0.45 (1.03)&0.21 (0.64)&31.17 (75.96)&39.00 (114.84)&5.24 (22.85)&4.92 (17.02)\\
/\periodic/\optavg/\mft[600]&0.45 (1.04)&0.21 (0.64)&31.23 (75.96)&38.96 (113.40)&5.24 (22.90)&4.92 (16.88)\\
/\periodic/\optavg/\mvt[300]&0.45 (1.02)&0.21 (0.63)&31.16 (75.24)&37.86 (111.24)&5.23 (22.16)&4.78 (16.52)\\
/\periodic/\optavg/\mvt[600]&0.45 (1.03)&0.20 (0.62)&31.04 (75.24)&36.62 (111.60)&5.20 (22.95)&4.63 (16.52)\\
/\periodic/\optmin&0.49 (1.07)&0.21 (0.62)&33.83 (84.24)&38.69 (111.24)&5.65 (23.23)&4.90 (16.58)\\
/\periodic/\optmin/\mft[300]&0.49 (1.07)&0.21 (0.62)&33.83 (84.24)&38.69 (111.24)&5.65 (23.23)&4.90 (16.58)\\
/\periodic/\optmin/\mft[600]&0.49 (1.07)&0.21 (0.62)&33.83 (84.24)&38.69 (111.24)&5.65 (23.23)&4.90 (16.58)\\
/\periodic/\optmin/\mvt[300]&0.49 (1.08)&0.20 (0.60)&33.88 (83.52)&37.62 (107.64)&5.65 (23.25)&4.77 (16.00)\\
/\periodic/\optmin/\mvt[600]&0.49 (1.08)&0.19 (0.58)&33.76 (84.60)&36.21 (104.04)&5.63 (22.78)&4.59 (15.51)\\
\mcbs/\periodic/\optavg&0.28 (0.66)&0.39 (0.79)&20.64 (43.20)&62.89 (140.04)&3.79 (16.03)&9.58 (23.98)\\
\mcbs/\periodic/\optavg/\mft[300]&0.28 (0.66)&0.39 (0.78)&20.65 (42.48)&63.03 (140.40)&3.79 (15.86)&9.60 (24.02)\\
\mcbs/\periodic/\optavg/\mft[600]&0.28 (0.66)&0.39 (0.78)&20.62 (43.56)&62.88 (138.96)&3.78 (16.13)&9.58 (23.79)\\
\mcbs/\periodic/\optavg/\mvt[300]&0.28 (0.68)&0.38 (0.79)&20.62 (43.20)&61.58 (136.80)&3.77 (16.24)&9.36 (23.27)\\
\mcbs/\periodic/\optavg/\mvt[600]&0.28 (0.68)&0.37 (0.78)&20.60 (43.56)&59.78 (132.48)&3.77 (16.00)&9.11 (22.63)\\
\mcbs/\periodic/\optmax&0.28 (0.65)&0.39 (0.81)&20.41 (45.36)&67.26 (159.48)&3.79 (16.71)&10.41 (26.96)\\
\mcbs/\periodic/\optmax/\mft[300]&0.28 (0.65)&0.39 (0.81)&20.41 (45.36)&67.26 (159.48)&3.79 (16.71)&10.41 (26.96)\\
\mcbs/\periodic/\optmax/\mft[600]&0.28 (0.65)&0.39 (0.81)&20.41 (45.36)&67.26 (159.48)&3.79 (16.71)&10.41 (26.96)\\
\mcbs/\periodic/\optmax/\mvt[300]&0.28 (0.65)&0.38 (0.81)&20.35 (46.44)&65.60 (158.40)&3.78 (17.13)&10.14 (26.75)\\
\mcbs/\periodic/\optmax/\mvt[600]&0.28 (0.64)&0.37 (0.78)&20.25 (46.80)&63.87 (153.36)&3.76 (17.52)&9.87 (25.78)\\


==> tabledata/deg-from-best-0-delay.tex <==
easy&1,529.0&1,702.1&10,153.3&1,875.0&963.5&4,451.5&1,962.1&899.5&4,573.4\\
fcfs&1,818.4&1,997.6&15,330.7&2,072.3&1,055.8&5,241.5&2,186.0&961.7&5,384.3\\
\greedy\activeres/opt=avg&520.2&1,044.6&7,464.0&944.4&874.8&3,491.7&1,242.9&943.3&6,175.9\\
\greedy\activeres/\periodic/opt=avg&6.8&6.8&23.9&8.6&4.9&20.0&8.7&4.1&27.1\\
\greedy\activeres/\periodic/opt=avg/mft=300&6.9&6.9&23.9&8.5&5.0&20.0&8.7&4.2&27.1\\
\greedy\activeres/\periodic/opt=avg/mft=600&6.9&6.8&23.9&8.5&4.8&20.0&8.7&4.2&27.1\\
\greedy\activeres/\periodic/opt=avg/mvt=300&6.9&6.9&23.9&8.7&4.8&20.0&8.7&4.2&27.1\\
\greedy\activeres/\periodic/opt=avg/mvt=600&7.0&6.8&23.9&8.8&4.9&20.0&8.7&4.1&27.1\\
\greedy\activeres/opt=min&500.2&993.1&7,257.1&928.5&855.7&3,618.0&1,207.4&927.0&6,315.5\\
\greedy\activeres/\periodic/opt=min&6.8&6.9&23.9&8.7&4.9&20.0&8.6&4.1&27.1\\
\greedy\activeres/\periodic/opt=min/mft=300&6.9&6.9&23.9&8.5&4.9&20.0&8.6&4.1&27.1\\
\greedy\activeres/\periodic/opt=min/mft=600&7.0&6.9&23.9&8.6&4.9&20.0&8.7&4.2&27.1\\
\greedy\activeres/\periodic/opt=min/mvt=300&6.9&6.9&23.9&8.6&4.8&20.0&8.7&4.1&27.1\\
\greedy\activeres/\periodic/opt=min/mvt=600&7.1&7.0&23.9&8.8&4.8&20.0&8.6&4.2&27.1\\
\greedy/\periodic/opt=avg&7.7&8.4&51.3&8.9&4.7&18.6&9.3&4.5&31.3\\
\greedy/\periodic/opt=avg/mft=300&7.6&8.3&51.3&8.9&4.7&18.6&9.2&4.5&31.3\\
\greedy/\periodic/opt=avg/mft=600&7.7&8.4&51.3&9.0&4.8&18.6&9.2&4.5&31.3\\
\greedy/\periodic/opt=avg/mvt=300&7.6&8.3&51.3&9.1&4.9&18.6&9.3&4.5&31.3\\
\greedy/\periodic/opt=avg/mvt=600&7.8&8.3&51.3&9.1&4.8&18.6&9.2&4.5&31.3\\
\greedy/\periodic/opt=min&7.7&8.3&51.3&9.1&4.8&18.6&9.3&4.5&31.3\\
\greedy/\periodic/opt=min/mft=300&7.7&8.3&51.3&8.8&4.8&18.6&9.2&4.5&31.3\\
\greedy/\periodic/opt=min/mft=600&7.4&8.2&51.3&9.0&5.0&18.6&9.2&4.5&31.3\\
\greedy/\periodic/opt=min/mvt=300&7.5&8.2&51.3&9.2&4.9&18.6&9.3&4.6&31.3\\
\greedy/\periodic/opt=min/mvt=600&7.7&8.3&51.3&9.2&4.9&18.6&9.3&4.6&31.3\\
\greedyp\activeres/opt=avg&5.1&29.2&285.3&9.2&33.0&202.4&35.2&196.8&2,596.4\\
\greedyp\activeres/\periodic/opt=avg&1.2&0.8&8.7&1.3&0.4&3.1&1.3&0.4&4.9\\
\greedyp\activeres/\periodic/opt=avg/mft=300&1.2&0.7&8.7&1.3&0.4&3.1&1.3&0.5&5.3\\
\greedyp\activeres/\periodic/opt=avg/mft=600&1.2&0.7&8.9&1.3&0.4&3.1&1.3&0.5&4.9\\
\greedyp\activeres/\periodic/opt=avg/mvt=300&1.2&0.8&8.9&1.3&0.4&3.1&1.3&0.5&4.9\\
\greedyp\activeres/\periodic/opt=avg/mvt=600&1.2&0.8&8.9&1.3&0.4&3.1&1.4&0.5&5.3\\
\greedyp\activeres/opt=min&4.9&28.3&274.9&12.0&53.2&461.5&36.9&196.7&2,544.5\\
\greedyp\activeres/\periodic/opt=min&1.2&0.7&8.7&1.2&0.3&3.1&1.3&0.4&4.9\\
\greedyp\activeres/\periodic/opt=min/mft=300&1.2&0.7&8.7&1.2&0.3&3.1&1.3&0.4&4.9\\
\greedyp\activeres/\periodic/opt=min/mft=600&1.2&0.7&8.7&1.2&0.3&3.1&1.3&0.4&4.9\\
\greedyp\activeres/\periodic/opt=min/mvt=300&1.2&0.7&8.7&1.2&0.3&3.1&1.3&0.4&4.9\\
\greedyp\activeres/\periodic/opt=min/mvt=600&1.2&0.7&8.7&1.2&0.4&3.2&1.3&0.4&4.9\\
\greedyp/\periodic/opt=avg&2.4&5.1&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedyp/\periodic/opt=avg/mft=300&2.5&5.2&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedyp/\periodic/opt=avg/mft=600&2.5&5.2&44.1&1.3&0.5&4.1&1.5&1.1&17.7\\
\greedyp/\periodic/opt=avg/mvt=300&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.1&17.7\\
\greedyp/\periodic/opt=avg/mvt=600&2.4&5.2&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedyp/\periodic/opt=min&2.5&5.2&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedyp/\periodic/opt=min/mft=300&2.4&5.1&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedyp/\periodic/opt=min/mft=600&2.4&5.2&44.1&1.3&0.5&4.1&1.4&1.1&17.7\\
\greedyp/\periodic/opt=min/mvt=300&2.4&5.2&44.1&1.3&0.5&4.1&1.4&1.1&17.7\\
\greedyp/\periodic/opt=min/mvt=600&2.4&5.2&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedypm\activeres/opt=avg&5.1&29.4&288.1&9.5&32.9&192.1&40.1&215.6&2,772.3\\
\greedypm\activeres/\periodic/opt=avg&1.2&0.8&8.7&1.3&0.4&3.1&1.3&0.4&4.9\\
\greedypm\activeres/\periodic/opt=avg/mft=300&1.2&0.7&8.7&1.3&0.4&3.2&1.3&0.5&4.9\\
\greedypm\activeres/\periodic/opt=avg/mft=600&1.2&0.7&8.9&1.3&0.4&3.1&1.3&0.5&5.3\\
\greedypm\activeres/\periodic/opt=avg/mvt=300&1.2&0.7&8.9&1.3&0.4&3.1&1.4&0.5&5.2\\
\greedypm\activeres/\periodic/opt=avg/mvt=600&1.2&0.7&8.9&1.3&0.4&3.2&1.4&0.5&5.2\\
\greedypm\activeres/opt=min&4.9&28.3&274.9&12.4&57.2&507.6&40.4&217.7&2,675.6\\
\greedypm\activeres/\periodic/opt=min&1.2&0.8&8.7&1.2&0.3&3.1&1.3&0.4&4.9\\
\greedypm\activeres/\periodic/opt=min/mft=300&1.2&0.8&8.7&1.2&0.3&3.1&1.3&0.4&4.9\\
\greedypm\activeres/\periodic/opt=min/mft=600&1.2&0.8&8.7&1.2&0.3&3.2&1.3&0.4&4.9\\
\greedypm\activeres/\periodic/opt=min/mvt=300&1.2&0.8&8.7&1.2&0.3&3.1&1.3&0.4&4.9\\
\greedypm\activeres/\periodic/opt=min/mvt=600&1.2&0.8&8.7&1.2&0.4&3.2&1.3&0.4&4.9\\
\greedypm/\periodic/opt=avg&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.0&17.7\\
\greedypm/\periodic/opt=avg/mft=300&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.0&17.7\\
\greedypm/\periodic/opt=avg/mft=600&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.0&17.7\\
\greedypm/\periodic/opt=avg/mvt=300&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.0&17.7\\
\greedypm/\periodic/opt=avg/mvt=600&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.0&17.7\\
\greedypm/\periodic/opt=min&2.3&4.9&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedypm/\periodic/opt=min/mft=300&2.4&5.1&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedypm/\periodic/opt=min/mft=600&2.4&5.1&44.1&1.3&0.5&4.1&1.4&1.0&17.7\\
\greedypm/\periodic/opt=min/mvt=300&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.1&17.7\\
\greedypm/\periodic/opt=min/mvt=600&2.4&5.1&44.1&1.3&0.5&4.1&1.5&1.0&17.7\\
\mcb\activeres/opt=avg&1.1&0.3&3.7&1.5&1.3&13.0&1.6&2.6&66.9\\
\mcb\activeres/opt=avg/mft=300&1.1&0.3&3.8&1.5&1.3&13.0&1.7&2.6&66.9\\
\mcb\activeres/opt=avg/mft=600&1.1&0.2&2.2&1.6&1.4&13.0&1.7&2.6&66.9\\
\mcb\activeres/opt=avg/mvt=300&1.1&0.5&5.6&1.5&1.3&12.9&1.7&2.5&66.9\\
\mcb\activeres/opt=avg/mvt=600&1.1&0.3&3.6&1.5&1.3&12.9&1.8&2.6&66.9\\
\mcb\activeres/\periodic/opt=avg&1.0&0.1&1.9&1.2&0.3&3.0&1.2&0.4&9.1\\
\mcb\activeres/\periodic/opt=avg/mft=300&1.1&0.2&3.8&1.2&0.3&3.2&1.3&0.4&9.1\\
\mcb\activeres/\periodic/opt=avg/mft=600&1.0&0.1&1.9&1.2&0.3&3.2&1.3&0.4&9.1\\
\mcb\activeres/\periodic/opt=avg/mvt=300&1.1&0.2&3.8&1.2&0.3&2.5&1.3&0.4&9.1\\
\mcb\activeres/\periodic/opt=avg/mvt=600&1.0&0.1&1.9&1.2&0.3&2.5&1.3&0.4&9.1\\
\mcb\activeres/opt=min&1.1&0.3&3.7&1.5&1.3&13.0&1.5&2.5&66.9\\
\mcb\activeres/opt=min/mft=300&1.1&0.4&5.6&1.5&1.3&13.0&1.6&2.6&66.9\\
\mcb\activeres/opt=min/mft=600&1.1&0.3&3.8&1.4&1.3&13.0&1.6&2.6&66.9\\
\mcb\activeres/opt=min/mvt=300&1.1&0.3&3.8&1.5&1.3&13.0&1.7&2.6&66.9\\
\mcb\activeres/opt=min/mvt=600&1.1&0.3&3.8&1.5&1.2&13.0&1.7&2.6&66.9\\
\mcb\activeres/\periodic/opt=min&1.0&0.1&1.9&1.1&0.2&1.9&1.1&0.4&9.1\\
\mcb\activeres/\periodic/opt=min/mft=300&1.1&0.2&3.8&1.1&0.2&1.9&1.2&0.4&9.1\\
\mcb\activeres/\periodic/opt=min/mft=600&1.1&0.2&3.8&1.1&0.2&2.0&1.2&0.4&9.1\\
\mcb\activeres/\periodic/opt=min/mvt=300&1.1&0.2&3.8&1.2&0.2&2.5&1.2&0.4&9.1\\
\mcb\activeres/\periodic/opt=min/mvt=600&1.1&0.2&3.8&1.2&0.2&2.5&1.3&0.4&9.1\\
\mcb/\periodic/opt=avg&1.9&3.5&36.9&1.2&0.2&2.2&1.3&0.4&3.9\\
\mcb/\periodic/opt=avg/mft=300&1.9&3.5&36.9&1.3&0.3&2.2&1.3&0.4&3.9\\
\mcb/\periodic/opt=avg/mft=600&1.9&3.5&36.9&1.2&0.3&2.2&1.3&0.4&3.9\\
\mcb/\periodic/opt=avg/mvt=300&1.9&3.5&36.9&1.3&0.3&2.5&1.4&0.4&3.9\\
\mcb/\periodic/opt=avg/mvt=600&1.9&3.5&36.9&1.3&0.3&2.5&1.4&0.4&3.9\\
\mcb/\periodic/opt=min&1.9&3.5&36.9&1.2&0.2&2.0&1.2&0.4&5.6\\
\mcb/\periodic/opt=min/mft=300&1.9&3.5&36.9&1.2&0.2&2.0&1.3&0.3&3.9\\
\mcb/\periodic/opt=min/mft=600&1.9&3.5&36.9&1.2&0.2&2.0&1.3&0.3&3.9\\
\mcb/\periodic/opt=min/mvt=300&1.9&3.5&36.9&1.2&0.2&2.5&1.3&0.4&3.9\\
\mcb/\periodic/opt=min/mvt=600&1.9&3.5&36.9&1.2&0.3&2.5&1.3&0.3&3.9\\
/\periodic/opt=avg&50.4&195.6&2,045.7&17.6&10.0&60.4&14.8&7.9&56.7\\
/\periodic/opt=avg/mft=300&50.4&195.6&2,045.7&17.6&10.0&60.4&14.7&7.9&56.7\\
/\periodic/opt=avg/mft=600&50.4&195.6&2,045.7&17.6&10.0&60.4&14.8&7.9&56.7\\
/\periodic/opt=avg/mvt=300&50.4&195.6&2,045.7&17.6&10.0&60.4&14.8&7.9&56.7\\
/\periodic/opt=avg/mvt=600&50.4&195.6&2,045.7&17.6&10.0&60.4&14.8&7.9&56.7\\
/\periodic/opt=min&50.4&195.6&2,045.7&17.6&10.0&60.4&14.7&7.9&56.7\\
/\periodic/opt=min/mft=300&50.4&195.6&2,045.7&17.6&10.0&60.4&14.7&7.9&56.7\\
/\periodic/opt=min/mft=600&50.4&195.6&2,045.7&17.6&10.0&60.4&14.7&7.9&56.7\\
/\periodic/opt=min/mvt=300&50.4&195.6&2,045.7&17.6&10.0&60.4&14.7&7.9&56.7\\
/\periodic/opt=min/mvt=600&50.4&195.6&2,045.7&17.6&10.0&60.4&14.8&7.9&56.7\\
\mcbs/opt=avg&50.3&195.6&2,045.7&17.5&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=avg/mft=300&50.3&195.6&2,045.7&17.5&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=avg/mft=600&50.3&195.6&2,045.7&17.5&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=avg/mvt=300&50.3&195.6&2,045.7&17.5&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=avg/mvt=600&50.3&195.6&2,045.7&17.5&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=max&50.3&195.6&2,045.7&17.4&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=max/mft=300&50.3&195.6&2,045.7&17.4&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=max/mft=600&50.3&195.6&2,045.7&17.4&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=max/mvt=300&50.3&195.6&2,045.7&17.5&10.0&60.5&14.6&7.9&56.7\\
\mcbs/opt=max/mvt=600&50.3&195.6&2,045.7&17.5&10.0&60.5&14.6&7.9&56.7\\


==> tabledata/deg-from-best-300-delay.tex <==
easy&1,145.2&1,482.7&9,350.7&1,375.8&663.4&2,959.0&1,320.3&665.6&3,959.4\\
fcfs&1,365.2&1,718.5&12,792.2&1,519.4&734.3&3,683.0&1,466.0&687.4&4,411.0\\
\greedy\activeres/opt=avg&359.0&859.7&6,316.7&666.9&632.6&3,022.1&806.0&611.0&4,388.2\\
\greedy\activeres/\periodic/opt=avg&9.2&6.5&30.6&9.7&4.5&30.8&7.7&3.8&24.2\\
\greedy\activeres/\periodic/opt=avg/mft=300&6.9&6.9&29.4&7.2&4.3&19.7&6.7&3.7&26.2\\
\greedy\activeres/\periodic/opt=avg/mft=600&6.7&6.7&27.0&7.0&4.2&19.7&6.4&3.7&20.1\\
\greedy\activeres/\periodic/opt=avg/mvt=300&6.7&6.6&25.7&7.1&4.3&19.7&6.5&3.7&20.1\\
\greedy\activeres/\periodic/opt=avg/mvt=600&6.6&6.7&30.0&6.9&4.1&19.7&6.4&3.7&20.1\\
\greedy\activeres/opt=min&337.1&771.8&5,886.7&646.3&604.5&3,047.2&781.2&604.7&4,388.2\\
\greedy\activeres/\periodic/opt=min&9.1&6.4&28.9&9.6&4.5&30.8&7.7&3.9&24.7\\
\greedy\activeres/\periodic/opt=min/mft=300&6.7&6.7&24.5&7.1&4.3&19.7&6.7&3.7&24.7\\
\greedy\activeres/\periodic/opt=min/mft=600&6.6&6.6&26.7&7.0&4.2&19.7&6.4&3.7&24.7\\
\greedy\activeres/\periodic/opt=min/mvt=300&6.5&6.4&23.5&7.0&4.2&19.7&6.4&3.7&20.1\\
\greedy\activeres/\periodic/opt=min/mvt=600&6.6&6.8&27.8&6.9&4.2&19.7&6.3&3.6&24.7\\
\greedy/\periodic/opt=avg&10.1&9.1&85.2&9.6&4.8&30.8&7.8&4.3&30.9\\
\greedy/\periodic/opt=avg/mft=300&7.3&8.4&72.9&7.6&4.4&19.7&7.0&4.3&30.9\\
\greedy/\periodic/opt=avg/mft=600&7.5&9.4&84.9&7.3&4.3&19.7&7.0&4.3&30.8\\
\greedy/\periodic/opt=avg/mvt=300&7.5&8.5&72.9&7.3&4.3&19.7&7.0&4.5&34.3\\
\greedy/\periodic/opt=avg/mvt=600&7.5&9.1&72.9&7.3&4.2&19.7&7.0&4.4&30.9\\
\greedy/\periodic/opt=min&9.8&8.4&78.8&9.6&4.8&30.8&7.8&4.4&30.9\\
\greedy/\periodic/opt=min/mft=300&7.3&7.9&60.8&7.4&4.3&19.7&7.0&4.3&30.9\\
\greedy/\periodic/opt=min/mft=600&7.3&7.8&61.0&7.4&4.3&19.7&7.0&4.5&34.3\\
\greedy/\periodic/opt=min/mvt=300&7.4&8.4&73.1&7.4&4.3&19.7&7.1&4.5&31.0\\
\greedy/\periodic/opt=min/mvt=600&7.1&7.7&60.8&7.4&4.3&19.7&6.9&4.3&30.9\\
\greedyp\activeres/opt=avg&2.2&5.7&60.0&7.8&39.2&357.1&19.3&109.5&1,724.7\\
\greedyp\activeres/\periodic/opt=avg&6.2&4.4&19.8&6.9&4.6&30.8&5.0&3.2&24.2\\
\greedyp\activeres/\periodic/opt=avg/mft=300&1.9&1.6&16.6&1.6&0.7&5.3&1.7&0.9&18.7\\
\greedyp\activeres/\periodic/opt=avg/mft=600&1.8&1.6&16.6&1.5&0.6&5.3&1.6&1.0&18.7\\
\greedyp\activeres/\periodic/opt=avg/mvt=300&1.7&1.1&11.7&1.4&0.6&5.0&1.5&1.0&18.7\\
\greedyp\activeres/\periodic/opt=avg/mvt=600&1.7&1.1&11.7&1.4&0.6&5.0&1.4&1.0&18.7\\
\greedyp\activeres/opt=min&1.9&3.7&40.1&9.0&40.8&349.6&19.3&111.6&1,736.8\\
\greedyp\activeres/\periodic/opt=min&6.2&4.3&19.8&6.9&4.6&30.8&4.9&3.2&24.2\\
\greedyp\activeres/\periodic/opt=min/mft=300&1.9&1.6&16.6&1.5&0.6&5.3&1.6&1.0&18.7\\
\greedyp\activeres/\periodic/opt=min/mft=600&1.7&1.5&16.6&1.4&0.7&5.3&1.5&0.8&18.7\\
\greedyp\activeres/\periodic/opt=min/mvt=300&1.7&1.1&11.7&1.4&0.6&5.1&1.4&0.8&18.7\\
\greedyp\activeres/\periodic/opt=min/mvt=600&1.6&1.1&11.7&1.4&0.7&5.1&1.4&1.0&18.7\\
\greedyp/\periodic/opt=avg&6.2&4.4&19.8&6.8&4.7&30.8&4.9&3.3&24.2\\
\greedyp/\periodic/opt=avg/mft=300&2.0&1.8&17.1&1.7&0.8&6.6&1.8&1.2&14.0\\
\greedyp/\periodic/opt=avg/mft=600&1.9&1.8&17.1&1.7&0.8&6.6&1.7&1.1&14.0\\
\greedyp/\periodic/opt=avg/mvt=300&2.0&1.8&17.1&1.7&0.8&5.3&1.7&1.2&14.0\\
\greedyp/\periodic/opt=avg/mvt=600&1.9&1.8&17.1&1.6&0.8&6.6&1.6&1.2&14.0\\
\greedyp/\periodic/opt=min&6.2&4.3&19.8&6.8&4.7&30.8&4.8&3.3&24.2\\
\greedyp/\periodic/opt=min/mft=300&2.0&1.8&17.1&1.7&0.7&5.3&1.7&1.2&14.0\\
\greedyp/\periodic/opt=min/mft=600&1.9&1.8&17.1&1.6&0.8&6.6&1.7&1.1&14.0\\
\greedyp/\periodic/opt=min/mvt=300&1.9&1.8&17.1&1.6&0.7&4.8&1.6&1.1&14.0\\
\greedyp/\periodic/opt=min/mvt=600&1.9&1.8&17.1&1.6&0.8&6.6&1.6&1.2&14.0\\
\greedypm\activeres/opt=avg&1.9&3.9&42.4&6.4&24.0&147.9&21.5&119.5&1,651.7\\
\greedypm\activeres/\periodic/opt=avg&6.2&4.4&19.8&6.9&4.6&30.8&5.0&3.2&24.2\\
\greedypm\activeres/\periodic/opt=avg/mft=300&1.9&1.7&19.5&1.6&0.7&5.3&1.7&0.7&9.0\\
\greedypm\activeres/\periodic/opt=avg/mft=600&1.8&1.7&19.5&1.4&0.6&5.3&1.6&1.1&18.7\\
\greedypm\activeres/\periodic/opt=avg/mvt=300&1.7&1.2&13.1&1.4&0.6&5.0&1.5&0.8&18.7\\
\greedypm\activeres/\periodic/opt=avg/mvt=600&1.7&1.2&13.1&1.4&0.6&5.0&1.5&1.1&18.7\\
\greedypm\activeres/opt=min&1.9&3.7&40.1&8.1&41.5&383.5&21.2&123.5&1,761.7\\
\greedypm\activeres/\periodic/opt=min&6.2&4.4&19.8&6.8&4.7&30.8&4.9&3.2&24.2\\
\greedypm\activeres/\periodic/opt=min/mft=300&1.9&1.7&19.5&1.5&0.7&5.3&1.6&1.0&18.7\\
\greedypm\activeres/\periodic/opt=min/mft=600&1.8&1.7&19.5&1.4&0.6&5.3&1.5&1.0&18.7\\
\greedypm\activeres/\periodic/opt=min/mvt=300&1.7&1.2&13.1&1.4&0.6&5.1&1.4&0.8&18.7\\
\greedypm\activeres/\periodic/opt=min/mvt=600&1.6&1.2&13.1&1.4&0.6&5.1&1.4&0.8&18.7\\
\greedypm/\periodic/opt=avg&6.2&4.4&19.8&6.8&4.7&30.8&4.9&3.3&24.2\\
\greedypm/\periodic/opt=avg/mft=300&2.0&1.8&17.1&1.8&0.7&4.8&1.8&1.1&14.0\\
\greedypm/\periodic/opt=avg/mft=600&1.9&1.8&17.1&1.7&0.7&6.6&1.7&1.1&14.0\\
\greedypm/\periodic/opt=avg/mvt=300&1.9&1.8&17.1&1.7&0.8&6.6&1.7&1.1&14.0\\
\greedypm/\periodic/opt=avg/mvt=600&1.9&1.8&17.1&1.6&0.8&6.6&1.6&1.1&14.0\\
\greedypm/\periodic/opt=min&6.2&4.3&19.8&6.8&4.7&30.8&4.9&3.3&24.2\\
\greedypm/\periodic/opt=min/mft=300&2.0&1.8&17.1&1.7&0.6&4.8&1.7&1.1&14.0\\
\greedypm/\periodic/opt=min/mft=600&1.9&1.8&17.1&1.6&0.8&6.6&1.7&1.1&14.0\\
\greedypm/\periodic/opt=min/mvt=300&1.9&1.7&17.1&1.6&0.7&5.3&1.6&1.1&14.0\\
\greedypm/\periodic/opt=min/mvt=600&1.8&1.8&17.1&1.6&0.8&6.6&1.6&1.1&14.0\\
\mcb\activeres/opt=avg&136.2&528.6&5,359.9&82.8&63.4&368.9&192.1&289.8&1,917.8\\
\mcb\activeres/opt=avg/mft=300&12.7&51.2&536.9&5.0&4.8&36.1&26.9&75.4&902.4\\
\mcb\activeres/opt=avg/mft=600&4.2&4.8&40.1&2.8&1.3&8.1&7.2&18.5&296.5\\
\mcb\activeres/opt=avg/mvt=300&3.7&4.0&26.4&2.5&1.3&8.1&3.5&4.4&51.9\\
\mcb\activeres/opt=avg/mvt=600&2.9&2.8&22.1&2.2&1.8&12.8&3.1&6.7&154.2\\
\mcb\activeres/\periodic/opt=avg&154.3&666.4&7,144.8&83.8&59.6&337.6&244.6&385.7&2,620.2\\
\mcb\activeres/\periodic/opt=avg/mft=300&16.2&75.7&917.2&5.4&6.7&61.2&37.2&113.8&1,367.5\\
\mcb\activeres/\periodic/opt=avg/mft=600&5.2&7.7&79.6&3.1&1.5&7.4&8.5&25.1&348.2\\
\mcb\activeres/\periodic/opt=avg/mvt=300&4.4&4.3&26.4&2.6&1.1&7.0&3.4&3.4&41.4\\
\mcb\activeres/\periodic/opt=avg/mvt=600&3.6&3.4&20.4&2.2&1.0&8.3&2.7&2.8&29.1\\
\mcb\activeres/opt=min&136.1&536.1&5,467.5&79.5&63.1&389.1&190.4&291.0&1,919.3\\
\mcb\activeres/opt=min/mft=300&12.3&44.6&374.2&4.6&4.5&36.1&25.7&76.3&920.1\\
\mcb\activeres/opt=min/mft=600&4.1&4.6&40.1&2.8&1.7&10.7&6.9&15.6&219.9\\
\mcb\activeres/opt=min/mvt=300&3.7&4.0&28.7&2.7&1.8&12.0&3.6&4.6&51.9\\
\mcb\activeres/opt=min/mvt=600&2.9&2.8&22.1&1.9&1.1&8.2&2.9&4.1&51.9\\
\mcb\activeres/\periodic/opt=min&152.5&650.2&6,925.4&83.7&63.3&389.1&243.3&390.9&2,533.2\\
\mcb\activeres/\periodic/opt=min/mft=300&16.1&72.6&862.1&5.2&6.6&61.2&35.1&101.7&1,054.7\\
\mcb\activeres/\periodic/opt=min/mft=600&5.3&7.6&73.8&3.1&1.5&7.4&8.1&22.5&307.5\\
\mcb\activeres/\periodic/opt=min/mvt=300&4.3&4.2&28.7&2.7&1.1&7.0&3.4&3.5&43.1\\
\mcb\activeres/\periodic/opt=min/mvt=600&3.6&3.3&19.0&2.3&1.1&6.8&2.8&3.3&43.1\\
\mcb/\periodic/opt=avg&69.9&295.5&3,353.2&45.8&32.7&196.3&41.6&36.1&314.3\\
\mcb/\periodic/opt=avg/mft=300&4.0&8.4&93.2&4.4&4.2&30.3&5.5&5.5&48.2\\
\mcb/\periodic/opt=avg/mft=600&2.9&2.7&19.8&2.9&1.8&11.5&3.7&3.8&43.7\\
\mcb/\periodic/opt=avg/mvt=300&2.8&2.4&17.2&2.6&1.2&9.0&2.9&2.5&39.6\\
\mcb/\periodic/opt=avg/mvt=600&2.5&2.0&17.2&2.3&1.2&9.3&2.6&2.7&39.6\\
\mcb/\periodic/opt=min&68.8&289.3&3,344.9&45.5&32.6&196.3&40.7&34.7&314.4\\
\mcb/\periodic/opt=min/mft=300&4.0&8.7&103.2&4.2&4.1&30.3&5.2&5.0&48.2\\
\mcb/\periodic/opt=min/mft=600&2.9&2.7&19.8&2.9&1.6&11.5&3.5&3.5&43.7\\
\mcb/\periodic/opt=min/mvt=300&2.9&2.4&17.2&2.6&1.2&9.0&3.0&3.5&69.3\\
\mcb/\periodic/opt=min/mvt=600&2.5&2.0&17.2&2.3&1.2&9.3&2.6&2.7&39.6\\
/\periodic/opt=avg&43.4&192.9&2,004.8&14.4&10.3&60.4&10.8&7.4&48.3\\
/\periodic/opt=avg/mft=300&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.4&48.3\\
/\periodic/opt=avg/mft=600&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.4&48.3\\
/\periodic/opt=avg/mvt=300&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.4&48.3\\
/\periodic/opt=avg/mvt=600&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.4&48.3\\
/\periodic/opt=min&43.4&192.9&2,004.8&14.4&10.3&60.4&10.8&7.4&48.3\\
/\periodic/opt=min/mft=300&43.4&192.9&2,004.8&14.4&10.3&60.4&10.8&7.4&48.3\\
/\periodic/opt=min/mft=600&43.4&192.9&2,004.8&14.4&10.3&60.4&10.8&7.4&48.3\\
/\periodic/opt=min/mvt=300&43.4&192.9&2,004.8&14.4&10.3&60.4&10.8&7.4&48.3\\
/\periodic/opt=min/mvt=600&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.4&48.3\\
\mcbs/opt=avg&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.4\\
\mcbs/opt=avg/mft=300&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.4\\
\mcbs/opt=avg/mft=600&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.4\\
\mcbs/opt=avg/mvt=300&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.4\\
\mcbs/opt=avg/mvt=600&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.3\\
\mcbs/opt=max&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.3\\
\mcbs/opt=max/mft=300&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.3\\
\mcbs/opt=max/mft=600&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.3\\
\mcbs/opt=max/mvt=300&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.3\\
\mcbs/opt=max/mvt=600&43.4&192.9&2,004.8&14.4&10.2&60.4&10.8&7.3&48.4\\


==> tabledata/deg-from-bound-0-delay.tex <==
easy&3,041.9&3,438.0&21,317.4&4,955.4&2,730.6&14,036.8&5,262.0&2,588.9&14,534.1\\
fcfs&3,578.5&3,727.8&21,718.4&5,457.2&2,958.5&15,102.7&5,869.3&2,789.1&17,403.3\\
\greedy\activeres/opt=avg&984.5&1,900.6&12,114.2&2,477.3&2,311.2&10,386.1&3,305.9&2,564.9&18,706.3\\
\greedy\activeres/\periodic/opt=avg&14.0&14.5&57.2&22.5&13.0&53.3&23.9&12.9&101.4\\
\greedy\activeres/\periodic/opt=avg/mft=300&14.2&14.6&56.2&22.5&13.5&53.3&24.1&13.2&101.4\\
\greedy\activeres/\periodic/opt=avg/mft=600&14.1&14.4&57.0&22.3&13.0&53.3&24.0&13.1&101.4\\
\greedy\activeres/\periodic/opt=avg/mvt=300&14.2&14.5&57.2&23.2&13.4&53.3&24.1&13.1&101.4\\
\greedy\activeres/\periodic/opt=avg/mvt=600&14.2&14.2&57.0&23.2&13.3&53.3&24.0&13.0&101.4\\
\greedy\activeres/opt=min&949.8&1,828.5&11,778.4&2,435.0&2,285.6&11,229.9&3,204.3&2,517.5&19,129.2\\
\greedy\activeres/\periodic/opt=min&14.0&14.6&56.2&22.9&13.2&53.3&23.6&12.8&101.4\\
\greedy\activeres/\periodic/opt=min/mft=300&14.2&14.6&57.0&22.5&13.6&53.3&23.7&13.0&101.4\\
\greedy\activeres/\periodic/opt=min/mft=600&14.2&14.6&57.0&22.6&13.5&53.3&23.9&13.2&101.4\\
\greedy\activeres/\periodic/opt=min/mvt=300&14.1&14.5&57.0&22.8&13.3&53.3&23.9&13.0&101.4\\
\greedy\activeres/\periodic/opt=min/mvt=600&14.5&14.7&56.6&23.3&13.3&53.3&23.7&12.9&101.4\\
\greedy/\periodic/opt=avg&16.6&20.7&115.1&23.6&13.2&57.8&25.6&14.1&94.2\\
\greedy/\periodic/opt=avg/mft=300&16.4&20.5&115.1&23.6&13.4&57.8&25.4&13.8&89.9\\
\greedy/\periodic/opt=avg/mft=600&16.5&20.7&115.1&23.8&13.4&57.8&25.5&14.0&89.9\\
\greedy/\periodic/opt=avg/mvt=300&16.5&20.5&115.1&24.1&13.8&57.8&25.6&13.9&89.9\\
\greedy/\periodic/opt=avg/mvt=600&16.7&20.7&115.1&24.2&13.6&57.8&25.6&14.0&90.4\\
\greedy/\periodic/opt=min&16.6&20.6&115.1&24.0&13.3&57.9&25.6&14.0&94.2\\
\greedy/\periodic/opt=min/mft=300&16.5&20.5&115.1&23.3&13.2&57.9&25.4&13.8&89.9\\
\greedy/\periodic/opt=min/mft=600&16.1&20.4&115.1&23.8&13.8&58.0&25.5&13.9&89.9\\
\greedy/\periodic/opt=min/mvt=300&16.3&20.6&115.1&24.3&13.6&57.9&25.5&14.0&89.9\\
\greedy/\periodic/opt=min/mvt=600&16.5&20.7&115.1&24.3&13.7&58.0&25.6&14.3&121.9\\
\greedyp\activeres/opt=avg&11.0&68.9&846.5&27.6&100.5&608.1&105.8&602.5&9,605.2\\
\greedyp\activeres/\periodic/opt=avg&2.6&2.6&25.8&3.3&1.1&6.9&3.6&1.5&14.5\\
\greedyp\activeres/\periodic/opt=avg/mft=300&2.6&2.6&25.8&3.3&1.2&8.2&3.6&1.5&14.5\\
\greedyp\activeres/\periodic/opt=avg/mft=600&2.6&2.6&26.3&3.3&1.2&8.9&3.7&1.6&14.5\\
\greedyp\activeres/\periodic/opt=avg/mvt=300&2.6&2.7&26.3&3.3&1.2&8.0&3.7&1.6&14.5\\
\greedyp\activeres/\periodic/opt=avg/mvt=600&2.6&2.7&26.3&3.3&1.2&6.9&3.7&1.6&14.5\\
\greedyp\activeres/opt=min&10.6&65.3&792.4&34.6&146.4&1,200.4&111.3&611.2&10,391.0\\
\greedyp\activeres/\periodic/opt=min&2.6&2.5&25.8&3.1&1.1&8.7&3.6&1.4&14.5\\
\greedyp\activeres/\periodic/opt=min/mft=300&2.6&2.5&25.8&3.1&1.0&8.2&3.6&1.5&14.5\\
\greedyp\activeres/\periodic/opt=min/mft=600&2.6&2.5&25.8&3.1&1.1&8.2&3.6&1.4&14.5\\
\greedyp\activeres/\periodic/opt=min/mvt=300&2.6&2.5&25.8&3.2&1.0&6.9&3.6&1.5&14.5\\
\greedyp\activeres/\periodic/opt=min/mvt=600&2.6&2.5&25.8&3.2&1.1&8.1&3.6&1.5&14.5\\
\greedyp/\periodic/opt=avg&5.6&13.1&97.7&3.4&1.4&11.2&4.0&3.7&75.5\\
\greedyp/\periodic/opt=avg/mft=300&5.8&13.5&97.7&3.4&1.5&11.2&4.0&4.2&75.5\\
\greedyp/\periodic/opt=avg/mft=600&5.8&13.4&97.7&3.4&1.5&11.2&4.2&4.3&75.5\\
\greedyp/\periodic/opt=avg/mvt=300&5.6&13.1&97.7&3.4&1.5&11.2&4.1&4.2&75.5\\
\greedyp/\periodic/opt=avg/mvt=600&5.7&13.2&97.7&3.4&1.5&11.2&4.1&4.2&75.5\\
\greedyp/\periodic/opt=min&5.7&13.2&97.7&3.3&1.4&11.2&3.8&3.7&75.5\\
\greedyp/\periodic/opt=min/mft=300&5.6&13.1&97.7&3.3&1.4&11.2&3.9&4.2&75.5\\
\greedyp/\periodic/opt=min/mft=600&5.7&13.2&97.7&3.3&1.5&11.2&4.0&4.2&75.5\\
\greedyp/\periodic/opt=min/mvt=300&5.6&13.2&97.7&3.3&1.4&11.2&4.0&4.3&75.5\\
\greedyp/\periodic/opt=min/mvt=600&5.6&13.2&97.7&3.3&1.4&11.2&4.0&4.2&75.5\\
\greedypm\activeres/opt=avg&11.0&69.4&854.7&28.3&98.9&577.1&119.5&641.4&8,568.3\\
\greedypm\activeres/\periodic/opt=avg&2.7&2.7&25.8&3.3&1.2&8.8&3.7&1.6&14.5\\
\greedypm\activeres/\periodic/opt=avg/mft=300&2.6&2.6&25.8&3.3&1.2&8.1&3.7&1.6&14.5\\
\greedypm\activeres/\periodic/opt=avg/mft=600&2.6&2.6&26.3&3.2&1.2&8.3&3.7&1.6&14.5\\
\greedypm\activeres/\periodic/opt=avg/mvt=300&2.6&2.6&26.3&3.2&1.1&6.9&3.7&1.7&19.9\\
\greedypm\activeres/\periodic/opt=avg/mvt=600&2.6&2.5&26.3&3.3&1.2&8.3&3.7&1.6&15.0\\
\greedypm\activeres/opt=min&10.6&65.3&792.4&35.6&156.7&1,320.5&120.9&658.3&9,551.2\\
\greedypm\activeres/\periodic/opt=min&2.6&2.6&25.8&3.1&1.1&8.8&3.6&1.4&14.5\\
\greedypm\activeres/\periodic/opt=min/mft=300&2.6&2.6&25.8&3.2&1.1&8.3&3.6&1.5&14.5\\
\greedypm\activeres/\periodic/opt=min/mft=600&2.6&2.6&25.8&3.1&1.1&8.1&3.6&1.5&14.5\\
\greedypm\activeres/\periodic/opt=min/mvt=300&2.6&2.6&25.8&3.2&1.1&8.0&3.6&1.5&14.5\\
\greedypm\activeres/\periodic/opt=min/mvt=600&2.6&2.6&25.8&3.2&1.1&8.1&3.6&1.5&14.5\\
\greedypm/\periodic/opt=avg&5.6&13.2&97.7&3.4&1.4&11.2&4.0&3.7&75.5\\
\greedypm/\periodic/opt=avg/mft=300&5.6&13.2&97.7&3.4&1.5&11.2&4.1&4.2&75.5\\
\greedypm/\periodic/opt=avg/mft=600&5.6&13.2&97.7&3.4&1.5&11.2&4.2&4.2&75.5\\
\greedypm/\periodic/opt=avg/mvt=300&5.7&13.4&97.7&3.4&1.5&11.2&4.2&4.2&75.5\\
\greedypm/\periodic/opt=avg/mvt=600&5.6&13.2&97.7&3.4&1.4&11.2&4.2&4.3&75.5\\
\greedypm/\periodic/opt=min&5.4&12.9&97.7&3.3&1.4&11.2&3.9&3.7&75.5\\
\greedypm/\periodic/opt=min/mft=300&5.6&13.3&97.7&3.3&1.4&11.2&4.0&4.2&75.5\\
\greedypm/\periodic/opt=min/mft=600&5.6&13.4&97.7&3.3&1.4&11.2&4.0&4.2&75.5\\
\greedypm/\periodic/opt=min/mvt=300&5.6&13.4&97.7&3.3&1.4&11.2&4.1&4.2&75.5\\
\greedypm/\periodic/opt=min/mvt=600&5.6&13.4&97.7&3.3&1.4&11.2&4.1&4.3&75.5\\
\mcb\activeres/opt=avg&2.3&1.3&12.7&3.9&4.1&42.0&4.5&9.1&248.6\\
\mcb\activeres/opt=avg/mft=300&2.3&1.6&15.5&3.9&4.3&42.1&4.6&9.1&248.6\\
\mcb\activeres/opt=avg/mft=600&2.3&1.3&12.7&4.2&4.5&42.0&4.8&9.3&248.6\\
\mcb\activeres/opt=avg/mvt=300&2.4&1.7&15.5&4.1&4.3&42.0&4.7&9.0&248.6\\
\mcb\activeres/opt=avg/mvt=600&2.3&1.3&12.7&4.0&4.1&41.9&4.9&9.2&248.6\\
\mcb\activeres/\periodic/opt=avg&2.1&0.8&6.8&3.1&1.0&6.3&3.3&1.6&33.7\\
\mcb\activeres/\periodic/opt=avg/mft=300&2.2&1.3&15.5&3.1&1.0&6.7&3.4&1.6&33.7\\
\mcb\activeres/\periodic/opt=avg/mft=600&2.1&0.8&6.8&3.2&1.2&9.1&3.5&1.7&33.7\\
\mcb\activeres/\periodic/opt=avg/mvt=300&2.2&1.3&15.5&3.2&1.2&9.7&3.5&1.7&33.7\\
\mcb\activeres/\periodic/opt=avg/mvt=600&2.1&0.8&6.8&3.2&1.2&9.7&3.6&1.7&33.7\\
\mcb\activeres/opt=min&2.3&1.2&12.7&3.9&4.2&42.1&4.2&9.0&248.6\\
\mcb\activeres/opt=min/mft=300&2.3&1.6&15.5&3.9&4.3&42.1&4.5&9.1&248.6\\
\mcb\activeres/opt=min/mft=600&2.3&1.6&15.5&3.9&4.3&42.1&4.6&9.2&248.6\\
\mcb\activeres/opt=min/mvt=300&2.3&1.6&15.5&4.0&4.3&42.1&4.7&9.2&248.6\\
\mcb\activeres/opt=min/mvt=600&2.3&1.6&15.5&3.9&4.1&42.1&4.7&9.1&248.6\\
\mcb\activeres/\periodic/opt=min&2.1&0.8&6.8&2.9&0.8&5.6&3.2&1.6&33.7\\
\mcb\activeres/\periodic/opt=min/mft=300&2.2&1.3&15.5&3.0&0.8&5.6&3.2&1.5&33.7\\
\mcb\activeres/\periodic/opt=min/mft=600&2.2&1.3&15.5&3.0&0.9&7.6&3.3&1.6&33.7\\
\mcb\activeres/\periodic/opt=min/mvt=300&2.2&1.3&15.5&3.0&1.1&9.7&3.4&1.6&33.7\\
\mcb\activeres/\periodic/opt=min/mvt=600&2.2&1.3&15.5&3.1&1.1&9.7&3.4&1.6&33.7\\
\mcb/\periodic/opt=avg&4.2&8.9&70.7&3.2&1.0&6.1&3.5&1.3&12.9\\
\mcb/\periodic/opt=avg/mft=300&4.3&9.2&70.7&3.3&1.1&6.5&3.6&1.4&12.9\\
\mcb/\periodic/opt=avg/mft=600&4.3&9.2&70.7&3.2&1.1&7.4&3.7&1.4&12.9\\
\mcb/\periodic/opt=avg/mvt=300&4.3&9.2&70.7&3.3&1.2&9.7&3.7&1.5&12.9\\
\mcb/\periodic/opt=avg/mvt=600&4.3&9.2&70.7&3.4&1.3&9.7&3.7&1.4&12.9\\
\mcb/\periodic/opt=min&4.2&8.9&70.7&3.0&0.9&6.6&3.3&1.3&16.8\\
\mcb/\periodic/opt=min/mft=300&4.3&9.2&70.7&3.1&0.9&6.0&3.4&1.3&12.9\\
\mcb/\periodic/opt=min/mft=600&4.3&9.2&70.7&3.1&1.0&7.6&3.5&1.4&12.9\\
\mcb/\periodic/opt=min/mvt=300&4.3&9.2&70.7&3.1&1.1&9.7&3.6&1.4&12.9\\
\mcb/\periodic/opt=min/mvt=600&4.3&9.2&70.7&3.2&1.2&9.7&3.6&1.4&12.9\\
/\periodic/opt=avg&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.1&238.3\\
/\periodic/opt=avg/mft=300&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.0&238.3\\
/\periodic/opt=avg/mft=600&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.0&238.3\\
/\periodic/opt=avg/mvt=300&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&24.9&238.3\\
/\periodic/opt=avg/mvt=600&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&24.9&238.3\\
/\periodic/opt=min&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.1&238.3\\
/\periodic/opt=min/mft=300&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.1&238.3\\
/\periodic/opt=min/mft=600&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.1&238.3\\
/\periodic/opt=min/mvt=300&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.0&238.3\\
/\periodic/opt=min/mvt=600&105.0&445.6&5,011.9&42.9&19.8&134.7&40.3&25.0&238.3\\
\mcbs/opt=avg&104.8&445.6&5,011.9&42.6&19.7&134.7&39.8&24.9&236.5\\
\mcbs/opt=avg/mft=300&104.8&445.6&5,011.9&42.6&19.7&134.7&39.8&24.9&236.5\\
\mcbs/opt=avg/mft=600&104.8&445.6&5,011.9&42.6&19.7&134.7&39.8&24.9&236.5\\
\mcbs/opt=avg/mvt=300&104.8&445.6&5,011.9&42.6&19.7&134.7&39.9&24.9&236.5\\
\mcbs/opt=avg/mvt=600&104.8&445.6&5,011.9&42.6&19.7&134.7&39.9&24.9&236.5\\
\mcbs/opt=max&104.8&445.6&5,011.9&42.6&19.7&134.7&39.8&24.9&236.9\\
\mcbs/opt=max/mft=300&104.8&445.6&5,011.9&42.6&19.7&134.7&39.8&24.9&236.9\\
\mcbs/opt=max/mft=600&104.8&445.6&5,011.9&42.6&19.7&134.7&39.8&24.9&236.9\\
\mcbs/opt=max/mvt=300&104.8&445.6&5,011.9&42.6&19.7&134.7&39.9&24.9&236.9\\
\mcbs/opt=max/mvt=600&104.8&445.6&5,011.9&42.6&19.7&134.7&39.9&24.9&236.9\\


==> tabledata/deg-from-bound-300-delay.tex <==
FCFS&3,578.5&3,727.8&21,718.4&5,457.2&2,958.5&15,102.7&5,869.3&2,789.1&17,403.3\\
EASY&3,041.9&3,438.0&21,317.4&4,955.4&2,730.6&14,036.8&5,262.0&2,588.9&14,534.1\\
\greedy\activeres/\optavg&1,012.2&2,229.5&19,799.1&2,527.1&2,472.3&12,487.5&3,326.7&2,561.2&18,310.2\\
\greedy\activeres/\optmin&949.8&1,828.5&11,778.4&2,435.0&2,285.6&11,229.9&3,204.3&2,517.5&19,129.2\\
\greedy/\periodic/\optavg&28.9&27.0&212.9&30.0&10.2&58.1&29.2&14.3&153.2\\
\greedy/\periodic/\optavg/\mft[300]&23.3&26.9&182.3&26.5&14.4&58.1&27.4&15.5&153.2\\
\greedy/\periodic/\optavg/\mft[600]&23.5&27.6&212.2&25.6&14.2&57.8&27.3&15.5&152.6\\
\greedy/\periodic/\optavg/\mvt[300]&23.9&26.9&182.3&25.7&14.5&57.8&27.5&15.8&153.2\\
\greedy/\periodic/\optavg/\mvt[600]&23.8&27.8&182.3&25.5&14.2&57.8&27.4&15.9&153.0\\
\greedy/\periodic/\optmin&28.3&24.9&163.7&30.1&10.2&58.1&29.3&14.3&153.2\\
\greedy/\periodic/\optmin/\mft[300]&23.4&26.0&152.0&26.0&14.3&58.1&27.4&15.7&153.2\\
\greedy/\periodic/\optmin/\mft[600]&23.1&24.8&152.5&25.9&14.5&58.0&27.4&15.9&152.6\\
\greedy/\periodic/\optmin/\mvt[300]&23.5&26.9&182.8&25.9&14.5&57.9&27.6&15.9&153.4\\
\greedy/\periodic/\optmin/\mvt[600]&23.0&25.9&152.0&25.9&14.2&58.0&27.0&15.5&152.8\\
\greedy\activeres/\periodic/\optavg&24.5&15.9&81.6&30.5&9.8&65.7&29.2&11.9&101.4\\
\greedy\activeres/\periodic/\optavg/\mft[300]&19.8&17.8&85.6&25.6&14.4&58.7&26.7&13.6&87.1\\
\greedy\activeres/\periodic/\optavg/\mft[600]&19.3&17.6&85.6&25.0&14.3&57.5&25.5&13.2&95.2\\
\greedy\activeres/\periodic/\optavg/\mvt[300]&19.2&17.5&85.6&25.3&14.4&57.5&25.6&13.0&81.0\\
\greedy\activeres/\periodic/\optavg/\mvt[600]&18.9&17.3&74.9&24.7&14.1&54.1&25.4&13.1&95.2\\
\greedy\activeres/\periodic/\optmin&24.3&15.9&81.6&30.4&9.7&65.7&29.1&12.3&101.4\\
\greedy\activeres/\periodic/\optmin/\mft[300]&19.5&17.7&85.6&25.1&14.3&57.5&26.4&13.2&87.1\\
\greedy\activeres/\periodic/\optmin/\mft[600]&19.1&17.5&85.6&24.9&14.3&57.5&25.5&13.3&103.9\\
\greedy\activeres/\periodic/\optmin/\mvt[300]&18.9&17.2&85.6&24.9&14.2&54.1&25.4&13.0&81.0\\
\greedy\activeres/\periodic/\optmin/\mvt[600]&19.0&17.4&66.1&24.6&14.3&54.1&25.1&13.0&95.2\\
\greedyp\activeres/\optavg&20.4&116.7&1,254.2&32.7&146.9&1,230.9&114.3&617.3&9,490.0\\
\greedyp\activeres/\optmin&13.5&68.0&819.2&37.5&156.0&1,204.9&115.7&644.0&10,354.2\\
\greedyp/\periodic/\optavg&18.4&18.6&152.4&20.2&7.2&38.1&18.0&9.7&84.6\\
\greedyp/\periodic/\optavg/\mft[300]&9.1&18.8&152.4&6.3&4.3&38.1&7.7&7.9&84.6\\
\greedyp/\periodic/\optavg/\mft[600]&9.0&18.7&152.4&6.1&4.4&38.1&7.5&7.8&84.6\\
\greedyp/\periodic/\optavg/\mvt[300]&9.0&18.8&152.4&6.0&3.9&27.5&7.4&7.8&84.6\\
\greedyp/\periodic/\optavg/\mvt[600]&8.9&18.9&152.4&6.0&4.5&38.1&7.3&8.4&96.8\\
\greedyp/\periodic/\optmin&18.5&18.6&152.4&20.1&7.3&38.1&17.8&9.6&84.6\\
\greedyp/\periodic/\optmin/\mft[300]&9.1&18.8&152.4&6.1&3.8&27.5&7.6&7.9&84.6\\
\greedyp/\periodic/\optmin/\mft[600]&9.0&18.9&152.4&6.1&4.5&38.1&7.3&7.6&84.6\\
\greedyp/\periodic/\optmin/\mvt[300]&9.0&18.9&152.4&5.9&3.8&27.5&7.3&7.7&84.6\\
\greedyp/\periodic/\optmin/\mvt[600]&8.9&18.9&152.4&5.9&4.5&38.1&7.3&8.5&96.8\\
\greedyp\activeres/\periodic/\optavg&17.9&19.7&213.5&20.4&6.8&32.0&18.1&8.6&89.9\\
\greedyp\activeres/\periodic/\optavg/\mft[300]&8.2&19.4&213.5&5.5&2.8&18.0&7.1&5.6&90.2\\
\greedyp\activeres/\periodic/\optavg/\mft[600]&7.7&18.5&198.8&5.1&2.8&18.0&6.7&6.3&103.5\\
\greedyp\activeres/\periodic/\optavg/\mvt[300]&7.0&14.0&149.3&4.9&2.4&13.6&6.5&6.7&103.5\\
\greedyp\activeres/\periodic/\optavg/\mvt[600]&6.9&14.0&149.3&4.8&2.4&13.6&6.3&6.3&103.5\\
\greedyp\activeres/\periodic/\optmin&17.9&19.6&213.5&20.3&6.8&32.0&17.9&8.6&89.9\\
\greedyp\activeres/\periodic/\optmin/\mft[300]&7.9&19.0&213.5&5.2&2.4&13.7&6.8&6.4&103.5\\
\greedyp\activeres/\periodic/\optmin/\mft[600]&7.5&18.0&198.8&5.0&2.7&18.0&6.3&5.4&90.2\\
\greedyp\activeres/\periodic/\optmin/\mvt[300]&6.9&14.0&149.3&4.9&2.7&18.0&6.1&5.4&90.2\\
\greedyp\activeres/\periodic/\optmin/\mvt[600]&6.9&14.2&149.3&4.9&2.9&19.2&6.1&6.3&103.5\\
\greedypm\activeres/\optavg&14.1&72.7&880.1&28.2&104.4&676.2&124.9&658.4&9,404.5\\
\greedypm\activeres/\optmin&13.8&68.2&819.2&33.8&154.0&1,321.7&124.0&673.5&9,598.8\\
\greedypm/\periodic/\optavg&18.5&19.2&158.7&20.2&7.2&38.1&18.1&9.9&93.3\\
\greedypm/\periodic/\optavg/\mft[300]&9.1&19.4&158.7&6.3&3.7&27.5&7.8&7.5&84.6\\
\greedypm/\periodic/\optavg/\mft[600]&9.0&19.3&158.7&6.1&4.4&38.1&7.5&7.5&84.6\\
\greedypm/\periodic/\optavg/\mvt[300]&9.1&19.4&158.7&6.2&4.5&38.1&7.4&7.5&84.6\\
\greedypm/\periodic/\optavg/\mvt[600]&8.9&19.5&158.7&5.9&4.4&38.1&7.3&8.0&96.8\\
\greedypm/\periodic/\optmin&18.4&18.8&158.7&20.2&7.3&38.1&17.9&9.8&93.0\\
\greedypm/\periodic/\optmin/\mft[300]&9.2&19.2&158.7&6.1&3.6&27.5&7.6&7.4&84.6\\
\greedypm/\periodic/\optmin/\mft[600]&9.1&19.3&158.7&6.0&4.4&38.1&7.4&7.5&84.6\\
\greedypm/\periodic/\optmin/\mvt[300]&8.9&18.8&158.7&6.0&3.9&27.5&7.3&7.6&84.6\\
\greedypm/\periodic/\optmin/\mvt[600]&8.8&18.9&158.7&5.9&4.5&38.1&7.3&8.1&96.8\\
\greedypm\activeres/\periodic/\optavg&17.8&19.3&198.6&20.4&6.8&32.0&18.2&8.7&89.9\\
\greedypm\activeres/\periodic/\optavg/\mft[300]&8.2&19.1&198.6&5.5&2.6&13.7&7.1&5.2&80.1\\
\greedypm\activeres/\periodic/\optavg/\mft[600]&7.8&19.0&198.8&5.0&2.5&13.7&6.8&6.4&103.5\\
\greedypm\activeres/\periodic/\optavg/\mvt[300]&7.0&14.1&149.6&4.9&2.5&13.8&6.4&5.6&90.2\\
\greedypm\activeres/\periodic/\optavg/\mvt[600]&6.9&14.2&149.6&4.8&2.4&13.6&6.5&6.6&103.5\\
\greedypm\activeres/\periodic/\optmin&17.9&19.3&198.6&20.3&6.9&32.0&17.9&8.6&89.9\\
\greedypm\activeres/\periodic/\optmin/\mft[300]&8.1&19.2&198.6&5.3&2.7&18.0&6.9&6.5&103.5\\
\greedypm\activeres/\periodic/\optmin/\mft[600]&7.9&19.1&198.8&4.9&2.5&13.7&6.4&6.3&103.5\\
\greedypm\activeres/\periodic/\optmin/\mvt[300]&6.9&14.3&149.6&4.9&2.7&18.0&6.3&5.6&90.2\\
\greedypm\activeres/\periodic/\optmin/\mvt[600]&6.9&14.4&149.6&4.8&2.4&13.6&6.1&5.4&90.2\\
\mcb\activeres/\optavg&346.3&1,223.1&13,399.7&245.1&130.3&634.2&750.1&1,100.8&6,274.4\\
\mcb\activeres/\optavg/\mft[300]&44.7&144.2&1,082.8&18.0&23.2&206.3&121.9&351.2&3,609.6\\
\mcb\activeres/\optavg/\mft[600]&20.6&63.9&672.0&9.8&6.4&43.6&33.2&95.9&1,509.2\\
\mcb\activeres/\optavg/\mvt[300]&14.1&33.2&370.0&8.6&5.6&43.9&15.3&20.9&270.9\\
\mcb\activeres/\optavg/\mvt[600]&12.1&32.8&370.0&7.7&6.9&44.8&14.5&40.9&1,068.1\\
\mcb\activeres/\optmin&345.6&1,241.5&13,668.8&233.2&117.1&634.2&742.4&1,103.0&6,130.4\\
\mcb\activeres/\optmin/\mft[300]&44.7&138.4&1,126.3&16.6&22.8&206.3&117.8&358.4&3,680.3\\
\mcb\activeres/\optmin/\mft[600]&19.1&59.2&672.0&9.9&8.1&51.3&31.7&78.0&1,216.7\\
\mcb\activeres/\optmin/\mvt[300]&14.0&33.2&370.0&9.2&8.0&65.3&15.7&22.5&270.9\\
\mcb\activeres/\optmin/\mvt[600]&12.0&32.8&370.0&6.9&5.4&44.4&13.2&21.6&270.9\\
\mcb/\periodic/\optavg&171.4&702.4&8,383.0&134.7&57.1&324.1&155.8&122.8&913.3\\
\mcb/\periodic/\optavg/\mft[300]&15.0&33.5&279.3&15.2&18.7&173.0&23.5&26.0&231.5\\
\mcb/\periodic/\optavg/\mft[600]&12.1&26.9&292.4&10.2&8.1&65.7&15.8&19.2&231.4\\
\mcb/\periodic/\optavg/\mvt[300]&11.5&25.3&287.6&9.2&6.8&51.3&12.1&12.3&127.5\\
\mcb/\periodic/\optavg/\mvt[600]&10.7&25.2&287.6&8.2&7.0&53.3&11.1&12.6&127.5\\
\mcb/\periodic/\optmin&169.1&691.4&8,362.3&133.7&57.5&323.7&153.0&118.1&909.5\\
\mcb/\periodic/\optmin/\mft[300]&15.1&34.5&309.3&14.5&18.6&173.0&22.1&24.0&231.5\\
\mcb/\periodic/\optmin/\mft[600]&12.1&26.9&292.4&10.0&8.1&65.7&15.2&18.9&231.4\\
\mcb/\periodic/\optmin/\mvt[300]&11.5&25.3&287.6&9.0&6.7&51.3&12.3&14.2&223.0\\
\mcb/\periodic/\optmin/\mvt[600]&10.8&25.3&287.6&8.1&6.6&53.3&11.0&12.6&127.5\\
\mcb\activeres/\periodic/\optavg&394.5&1,562.9&17,862.0&252.1&126.3&634.2&959.5&1,469.0&8,299.4\\
\mcb\activeres/\periodic/\optavg/\mft[300]&56.1&197.4&1,849.6&19.5&35.4&349.2&168.2&516.8&5,469.8\\
\mcb\activeres/\periodic/\optavg/\mft[600]&23.6&71.3&799.3&10.7&5.6&37.1&40.3&155.5&2,941.5\\
\mcb\activeres/\periodic/\optavg/\mvt[300]&15.5&30.6&318.9&8.8&3.5&19.0&14.2&15.7&195.7\\
\mcb\activeres/\periodic/\optavg/\mvt[600]&13.7&30.3&318.9&7.8&3.8&21.4&12.0&14.5&195.7\\
\mcb\activeres/\periodic/\optmin&389.1&1,522.1&17,313.6&250.6&125.0&634.2&956.8&1,486.7&8,398.3\\
\mcb\activeres/\periodic/\optmin/\mft[300]&56.8&198.7&1,738.4&19.0&35.3&349.2&161.4&481.8&4,590.5\\
\mcb\activeres/\periodic/\optmin/\mft[600]&25.1&81.4&799.3&10.6&5.7&37.1&37.9&126.9&2,400.6\\
\mcb\activeres/\periodic/\optmin/\mvt[300]&15.4&30.6&318.9&8.9&3.5&19.0&14.4&17.4&222.2\\
\mcb\activeres/\periodic/\optmin/\mvt[600]&13.6&30.2&318.9&7.8&3.9&21.9&12.2&15.3&195.7\\
/\periodic/\optavg&105.0&445.6&5,011.9&43.1&19.7&134.7&40.4&25.1&238.3\\
/\periodic/\optavg/\mft[300]&105.0&445.6&5,011.9&43.0&19.7&134.7&40.4&25.0&238.3\\
/\periodic/\optavg/\mft[600]&105.0&445.6&5,011.9&43.0&19.7&134.7&40.4&25.1&238.3\\
/\periodic/\optavg/\mvt[300]&105.0&445.6&5,011.9&43.0&19.8&134.7&40.4&25.0&238.3\\
/\periodic/\optavg/\mvt[600]&105.0&445.6&5,011.9&43.1&19.7&134.7&40.4&25.0&238.3\\
/\periodic/\optmin&105.0&445.6&5,011.9&43.0&19.8&134.7&40.4&25.1&238.3\\
/\periodic/\optmin/\mft[300]&105.0&445.6&5,011.9&43.0&19.8&134.7&40.4&25.1&238.3\\
/\periodic/\optmin/\mft[600]&105.0&445.6&5,011.9&43.0&19.8&134.7&40.4&25.1&238.3\\
/\periodic/\optmin/\mvt[300]&105.0&445.6&5,011.9&43.0&19.8&134.7&40.4&25.0&238.3\\
/\periodic/\optmin/\mvt[600]&105.0&445.6&5,011.9&43.0&19.7&134.7&40.4&25.0&238.3\\
\mcbs/\periodic/\optavg&105.0&445.6&5,011.9&43.1&19.5&134.7&40.2&24.8&236.5\\
\mcbs/\periodic/\optavg/\mft[300]&105.0&445.6&5,011.9&43.1&19.5&134.7&40.2&24.8&236.5\\
\mcbs/\periodic/\optavg/\mft[600]&105.0&445.6&5,011.9&43.1&19.5&134.7&40.2&24.8&236.5\\
\mcbs/\periodic/\optavg/\mvt[300]&105.0&445.6&5,011.9&43.1&19.5&134.7&40.2&24.8&236.5\\
\mcbs/\periodic/\optavg/\mvt[600]&105.0&445.6&5,011.9&43.0&19.6&134.7&40.2&24.8&236.5\\
\mcbs/\periodic/\optmax&105.0&445.6&5,011.9&43.0&19.6&134.7&40.2&24.8&236.9\\
\mcbs/\periodic/\optmax/\mft[300]&105.0&445.6&5,011.9&43.0&19.6&134.7&40.2&24.8&236.9\\
\mcbs/\periodic/\optmax/\mft[600]&105.0&445.6&5,011.9&43.0&19.6&134.7&40.2&24.8&236.9\\
\mcbs/\periodic/\optmax/\mvt[300]&105.0&445.6&5,011.9&43.0&19.6&134.7&40.2&24.8&236.9\\
\mcbs/\periodic/\optmax/\mvt[600]&105.0&445.6&5,011.9&43.0&19.6&134.7&40.2&24.8&236.9\\

